Taylor-Lagrange Neural Ordinary Differential Equations: Toward Fast Training and Evaluation of Neural ODEs

Neural ordinary differential equations (NODEs) -- parametrizations of differential equations using neural networks -- have shown tremendous promise in learning models of unknown continuous-time dynamical systems from data. However, every forward evaluation of a NODE requires numerical integration of the neural network used to capture the system dynamics, making their training prohibitively expensive. Existing works rely on off-the-shelf adaptive step-size numerical integration schemes, which often require an excessive number of evaluations of the underlying dynamics network to obtain sufficient accuracy for training. By contrast, we accelerate the evaluation and the training of NODEs by proposing a data-driven approach to their numerical integration. The proposed Taylor-Lagrange NODEs (TL-NODEs) use a fixed-order Taylor expansion for numerical integration, while also learning to estimate the expansion's approximation error. As a result, the proposed approach achieves the same accuracy as adaptive step-size schemes while employing only low-order Taylor expansions, thus greatly reducing the computational cost necessary to integrate the NODE. A suite of numerical experiments, including modeling dynamical systems, image classification, and density estimation, demonstrate that TL-NODEs can be trained more than an order of magnitude faster than state-of-the-art approaches, without any loss in performance.

==> figs/mnist/mnist_plot.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0,1}

\begin{groupplot}[group style={group name = plots, group size=2 by 1, vertical sep=0.0cm, horizontal sep=2.0cm}]

\nextgroupplot[
width=0.5\textwidth, 
height=4.0cm,
tick align=inside,
legend cell align={left},
legend columns=3,
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1.1, 1.6)},
  anchor=north,
  draw=white!80!black
},
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Training steps},
xmajorgrids,
xmin=-11.95, xmax=250.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={NFE},
ymajorgrids,
ymin=40.1, ymax=125.9,
ytick style={color=black}
]

\input{figs/mnist/nfe_ode_data}

\nextgroupplot[
width=0.5\textwidth, 
height=4.0cm,
tick align=inside,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Training steps},
xmajorgrids,
xmin=-11.95, xmax=250.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Accuracy (\%)},
ymajorgrids,
ymin=0.95, ymax=0.99,
ytick style={color=black}
]

\input{figs/mnist/predaccuracy_data}

\end{groupplot}

\end{tikzpicture}

==> figs/mnist/nfe_ode.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,1,0}
\definecolor{color1}{rgb}{1,0,1}
\definecolor{color2}{rgb}{0,1,1}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.5,0.91)},
  anchor=north,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Training steps},
xmajorgrids,
xmin=-11.95, xmax=250.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Number of neural netowrk evaluation},
ymajorgrids,
ymin=40.1, ymax=125.9,
ytick style={color=black}
]
\addplot [thick, blue]
table {%
0 50
1 56
24 56
25 56.2999992370605
26 62
27 62
28 61.7000007629395
29 62
55 62
56 63.5
57 62
58 66.8000030517578
59 66.2000045776367
60 68
61 64.7000045776367
62 68
80 68
81 74
87 74
88 74.9000015258789
89 80
93 80
94 84.8000030517578
95 86
169 86
170 92
171 86
198 86
199 92
200 86
239 86
};
\addlegendentry{Tayla, p=2, H=2}
\addplot [thick, green!50.1960784313725!black]
table {%
0 44
1 44
2 50
7 50
8 44
18 44
19 50
59 50
60 50.6000022888184
61 50
62 50.2999992370605
63 50
65 50
66 53.9000015258789
67 56
68 50.9000015258789
69 51.2000007629395
70 50
71 55.7000007629395
72 56
74 56
76 55.4000015258789
77 56
239 56
};
\addlegendentry{Tayla, p=1, H=2}
\addplot [thick, color0]
table {%
0 50
2 50
3 56
6 56
7 50.9000015258789
8 50
14 50
15 50.6000022888184
16 56
41 56
42 57.2000007629395
43 59.2999992370605
44 62
90 62
91 62.2999992370605
92 62
93 68
94 62
95 65.9000015258789
96 64.7000045776367
97 68
99 68
100 62
104 62
105 63.5
106 62
109 62
110 64.7000045776367
111 62
114 62
115 62.9000015258789
116 62
117 67.4000015258789
118 62
127 62
128 65.9000015258789
129 62
239 62
};
\addlegendentry{Tayla, p=1, H=6}
\addplot [line width=2pt, color1]
table {%
0 95.5999984741211
239 95.5999984741211
};
\addlegendentry{RNODE}
\addplot [line width=2pt, color2]
table {%
0 80
239 80
};
\addlegendentry{TayNode}
\addplot [line width=2pt, white!50.1960784313725!black]
table {%
0 122
239 122
};
\addlegendentry{Vanilla NeuralODE}
\end{axis}

\end{tikzpicture}


==> figs/mnist/nfe_ode_data.tex <==
\definecolor{color0}{rgb}{1,1,0}
\definecolor{color1}{rgb}{1,0,1}
\definecolor{color2}{rgb}{0,1,1}

\addplot [thick, blue]
table {%
0 50
1 56
24 56
25 56.2999992370605
26 62
27 62
28 61.7000007629395
29 62
55 62
56 63.5
57 62
58 66.8000030517578
59 66.2000045776367
60 68
61 64.7000045776367
62 68
80 68
81 74
87 74
88 74.9000015258789
89 80
93 80
94 84.8000030517578
95 86
169 86
170 92
171 86
198 86
199 92
200 86
239 86
};
\addlegendentry{TLN, \(p=2\), \(H=2\)}
\addplot [thick, green!50.1960784313725!black]
table {%
0 44
1 44
2 50
7 50
8 44
18 44
19 50
59 50
60 50.6000022888184
61 50
62 50.2999992370605
63 50
65 50
66 53.9000015258789
67 56
68 50.9000015258789
69 51.2000007629395
70 50
71 55.7000007629395
72 56
74 56
76 55.4000015258789
77 56
239 56
};
\addlegendentry{TLN, \(p=1\), \(H=2\)}
\addplot [thick, color0]
table {%
0 50
2 50
3 56
6 56
7 50.9000015258789
8 50
14 50
15 50.6000022888184
16 56
41 56
42 57.2000007629395
43 59.2999992370605
44 62
90 62
91 62.2999992370605
92 62
93 68
94 62
95 65.9000015258789
96 64.7000045776367
97 68
99 68
100 62
104 62
105 63.5
106 62
109 62
110 64.7000045776367
111 62
114 62
115 62.9000015258789
116 62
117 67.4000015258789
118 62
127 62
128 65.9000015258789
129 62
239 62
};
\addlegendentry{TLN, \(p=1\), \(H=6\)}
\addplot [line width=2pt, color1]
table {%
0 95.5999984741211
239 95.5999984741211
};
\addlegendentry{RNODE}
\addplot [ultra thick, black, dashed]
table {%
0 80
239 80
};
\addlegendentry{TayNode}
\addplot [line width=2pt, white!50.1960784313725!black]
table {%
0 122
239 122
};
\addlegendentry{Vanilla NeuralODE}

==> figs/mnist/predaccuracy.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,1,0}
\definecolor{color1}{rgb}{1,0,1}
\definecolor{color2}{rgb}{0,1,1}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Training steps},
xmajorgrids,
xmin=-11.95, xmax=250.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Prediction accuracy (\%)},
ymajorgrids,
ymin=0.64182001054287, ymax=0.999979975819588,
ytick style={color=black}
]
\addplot [thick, blue]
table {%
0 0.658100008964539
1 0.803100109100342
2 0.867100238800049
3 0.89109992980957
4 0.905400276184082
5 0.90690016746521
6 0.911800026893616
7 0.909000158309937
8 0.919400215148926
9 0.921299934387207
10 0.92300009727478
11 0.918200135231018
12 0.928200006484985
13 0.92710018157959
14 0.932699918746948
15 0.936100125312805
16 0.942000150680542
17 0.940600156784058
18 0.945800065994263
19 0.939600110054016
20 0.947600126266479
21 0.954600095748901
22 0.951900005340576
23 0.951500177383423
24 0.956799983978271
25 0.954200029373169
26 0.959700107574463
27 0.956100106239319
28 0.959500074386597
29 0.965200066566467
30 0.964999914169312
31 0.957300186157227
32 0.964300155639648
33 0.966400146484375
34 0.963100075721741
35 0.960400104522705
36 0.96969997882843
37 0.968600034713745
38 0.968800067901611
39 0.972300171852112
40 0.970800042152405
41 0.968699932098389
42 0.969800114631653
43 0.970500111579895
44 0.970800042152405
45 0.967700004577637
46 0.972100019454956
47 0.972000122070312
48 0.972400188446045
49 0.969600200653076
50 0.969099998474121
51 0.970700025558472
52 0.969799995422363
53 0.969599962234497
54 0.973800182342529
55 0.974800109863281
56 0.970900058746338
57 0.976000070571899
58 0.972100019454956
59 0.970700025558472
60 0.975000143051147
61 0.974000215530396
62 0.97160005569458
63 0.976100206375122
64 0.97760009765625
65 0.971500039100647
66 0.976000070571899
67 0.974400043487549
68 0.973200082778931
69 0.977200150489807
70 0.975800037384033
71 0.973600029945374
72 0.976599931716919
73 0.975500106811523
74 0.975300073623657
75 0.978100061416626
76 0.977800130844116
77 0.973800182342529
78 0.978500127792358
79 0.971400022506714
80 0.973200082778931
81 0.975399971008301
82 0.978800296783447
83 0.976500153541565
84 0.975800156593323
85 0.974400162696838
86 0.974100112915039
87 0.97979998588562
88 0.979900121688843
89 0.977699995040894
90 0.979200005531311
91 0.97790002822876
92 0.972599983215332
93 0.974700093269348
94 0.977200150489807
95 0.978100061416626
96 0.976200103759766
97 0.975800156593323
98 0.976999998092651
99 0.976800084114075
100 0.978800058364868
101 0.979700088500977
102 0.978100061416626
104 0.980100154876709
105 0.980599999427795
106 0.976500034332275
107 0.980400085449219
108 0.979900002479553
109 0.979099988937378
110 0.976900100708008
111 0.979700088500977
112 0.976999998092651
113 0.980500221252441
114 0.977800130844116
115 0.978100061416626
116 0.979200005531311
117 0.981500148773193
118 0.977200031280518
119 0.980400204658508
120 0.981800079345703
121 0.982399940490723
122 0.977500081062317
123 0.981200218200684
124 0.981800079345703
125 0.981100082397461
126 0.98229992389679
127 0.981500148773193
128 0.980900049209595
129 0.982000112533569
130 0.980200052261353
131 0.981900215148926
132 0.980600118637085
133 0.982600212097168
134 0.980800151824951
135 0.981000065803528
136 0.980599999427795
137 0.982300043106079
138 0.982400059700012
139 0.980700016021729
140 0.981800079345703
141 0.981600046157837
142 0.98229992389679
143 0.982500195503235
144 0.982899904251099
145 0.982000112533569
146 0.981400012969971
147 0.981100082397461
148 0.983200073242188
150 0.981899976730347
152 0.982300043106079
153 0.98170018196106
154 0.982500076293945
155 0.981899976730347
156 0.982100129127502
158 0.981899976730347
159 0.981000065803528
160 0.981199979782104
161 0.980499982833862
162 0.983200073242188
163 0.981600046157837
165 0.981400012969971
166 0.982500076293945
167 0.98170006275177
168 0.982700109481812
169 0.982599973678589
170 0.979900121688843
171 0.982100009918213
173 0.982100009918213
174 0.979600071907043
175 0.982500076293945
176 0.982300043106079
177 0.98170006275177
178 0.983000040054321
179 0.981899976730347
180 0.982699990272522
181 0.982199907302856
182 0.983200073242188
183 0.981600046157837
184 0.981800079345703
185 0.982800006866455
186 0.982400059700012
187 0.983100056648254
188 0.98170018196106
189 0.981600046157837
190 0.98170006275177
191 0.981199979782104
193 0.982699990272522
194 0.980200052261353
195 0.982100009918213
196 0.982200145721436
197 0.981800079345703
198 0.983700037002563
199 0.981100082397461
200 0.983000040054321
201 0.982200145721436
202 0.982100009918213
203 0.981600046157837
204 0.982200145721436
205 0.983100056648254
206 0.982700109481812
207 0.981300115585327
208 0.982300043106079
209 0.981800079345703
210 0.982800126075745
211 0.982500076293945
212 0.982400059700012
213 0.981100082397461
214 0.979100227355957
215 0.982900142669678
216 0.982400178909302
219 0.982300043106079
220 0.978900074958801
221 0.98170006275177
222 0.982800006866455
223 0.982700109481812
224 0.982100009918213
225 0.982400059700012
226 0.981899976730347
227 0.981600046157837
228 0.983100056648254
229 0.983500123023987
230 0.982800006866455
231 0.982300043106079
232 0.982700109481812
233 0.98199999332428
234 0.98330020904541
235 0.983000040054321
236 0.983200073242188
237 0.982500076293945
238 0.978800058364868
239 0.982900142669678
};
\addlegendentry{Tayla, p=2, H=2}
\addplot [thick, green!50.1960784313725!black]
table {%
0 0.662699937820435
1 0.778600096702576
2 0.815700054168701
3 0.862900018692017
4 0.885699987411499
5 0.898200035095215
6 0.902200222015381
7 0.908099889755249
8 0.91349995136261
9 0.913400173187256
10 0.916800022125244
11 0.914799928665161
12 0.919800043106079
13 0.922100067138672
14 0.923400044441223
15 0.926700115203857
16 0.928499937057495
17 0.930800080299377
18 0.932000160217285
19 0.930999994277954
20 0.934900045394897
21 0.942600011825562
22 0.940000057220459
23 0.946500062942505
24 0.944400072097778
25 0.945500135421753
26 0.952100038528442
27 0.955300092697144
28 0.954400062561035
29 0.959200024604797
30 0.956500053405762
31 0.958400249481201
32 0.959200024604797
33 0.958700180053711
34 0.964900016784668
35 0.953200101852417
36 0.963299989700317
37 0.960400104522705
38 0.964800000190735
39 0.967600107192993
40 0.96779990196228
41 0.966500043869019
43 0.964400053024292
44 0.967400074005127
45 0.964100003242493
46 0.966300249099731
47 0.967900037765503
48 0.964299917221069
49 0.964699983596802
50 0.966399908065796
51 0.970299959182739
52 0.971699953079224
53 0.967900037765503
54 0.970599889755249
55 0.968400120735168
56 0.968199968338013
57 0.972300171852112
58 0.97379994392395
59 0.964400053024292
60 0.972100019454956
61 0.972000122070312
62 0.970400094985962
64 0.971400022506714
65 0.968900203704834
66 0.970500111579895
67 0.967200040817261
68 0.973900079727173
69 0.975100040435791
70 0.969300031661987
71 0.974700212478638
72 0.968600034713745
73 0.968800187110901
74 0.972100257873535
75 0.976000070571899
76 0.972399950027466
77 0.969000101089478
78 0.974200010299683
79 0.973600149154663
80 0.972500085830688
81 0.974600076675415
82 0.974499940872192
83 0.971100091934204
84 0.97540009021759
85 0.968400239944458
86 0.97570013999939
87 0.970999956130981
88 0.970700025558472
89 0.975899934768677
90 0.973000049591064
91 0.970300197601318
92 0.971900105476379
93 0.974999904632568
94 0.97350001335144
95 0.969500064849854
96 0.966799974441528
97 0.975500106811523
98 0.973100185394287
99 0.97350025177002
100 0.977500081062317
101 0.977500081062317
102 0.975600004196167
103 0.976900100708008
104 0.976600170135498
105 0.97790002822876
106 0.976500034332275
107 0.976999998092651
108 0.974000096321106
109 0.976900100708008
110 0.975900173187256
111 0.978400230407715
112 0.97790002822876
113 0.976900100708008
114 0.975600004196167
115 0.975800037384033
116 0.977999925613403
117 0.978700160980225
119 0.974800109863281
120 0.977800011634827
121 0.977200031280518
122 0.977200031280518
123 0.976700067520142
124 0.976999998092651
125 0.977699995040894
126 0.979099988937378
127 0.976500034332275
128 0.978300094604492
129 0.976999998092651
130 0.976999998092651
131 0.974699974060059
132 0.979399919509888
133 0.977699995040894
134 0.975100040435791
135 0.97760009765625
136 0.977099895477295
137 0.976099967956543
138 0.976500034332275
139 0.977800130844116
140 0.978500127792358
141 0.97760009765625
142 0.97700023651123
143 0.977499961853027
144 0.978500008583069
145 0.976400375366211
146 0.978200078010559
147 0.978000164031982
149 0.976700067520142
150 0.978100061416626
151 0.977800130844116
152 0.978800058364868
153 0.97790002822876
154 0.977800130844116
155 0.976700067520142
156 0.977499961853027
157 0.976900100708008
158 0.978400230407715
159 0.978300094604492
160 0.977299928665161
161 0.976800084114075
162 0.978200197219849
163 0.978900074958801
164 0.978800058364868
165 0.978100061416626
166 0.97790002822876
167 0.976400017738342
168 0.978900194168091
169 0.97790002822876
170 0.978399991989136
172 0.977800130844116
173 0.978100061416626
174 0.978700160980225
175 0.978000164031982
176 0.978500127792358
177 0.978200078010559
178 0.978300094604492
179 0.977900147438049
180 0.978900194168091
181 0.979300141334534
182 0.979000091552734
183 0.977299928665161
184 0.97790002822876
185 0.977299928665161
186 0.978100061416626
188 0.979000091552734
189 0.978700160980225
190 0.977499961853027
191 0.977699995040894
192 0.978800058364868
193 0.977100133895874
194 0.978899955749512
195 0.978000164031982
196 0.977500081062317
197 0.97730016708374
198 0.979200124740601
199 0.979800224304199
200 0.978800058364868
201 0.978000164031982
202 0.978500008583069
203 0.97790002822876
204 0.978900194168091
205 0.979000091552734
207 0.97790002822876
208 0.977100014686584
209 0.97760009765625
210 0.979200124740601
211 0.978400230407715
212 0.978600144386292
213 0.978200078010559
214 0.97760009765625
215 0.978899955749512
216 0.978700160980225
217 0.980000019073486
218 0.978100061416626
219 0.978600025177002
220 0.977299928665161
221 0.977400064468384
223 0.979099988937378
224 0.978800058364868
225 0.978300094604492
226 0.978600144386292
227 0.976699948310852
228 0.979400157928467
229 0.979099988937378
230 0.979200124740601
231 0.979000091552734
232 0.978200078010559
233 0.976399898529053
235 0.979900121688843
236 0.979400157928467
237 0.978500127792358
238 0.978700160980225
239 0.977200031280518
};
\addlegendentry{Tayla, p=1, H=2}
\addplot [thick, color0]
table {%
0 0.667799949645996
1 0.801800012588501
2 0.857600212097168
3 0.888700127601624
4 0.899900078773499
5 0.907000064849854
6 0.914499998092651
7 0.910700082778931
8 0.917700052261353
9 0.917900085449219
10 0.921600103378296
11 0.922199964523315
12 0.926300168037415
14 0.93120002746582
15 0.928300142288208
16 0.936599969863892
17 0.938600182533264
18 0.942999958992004
19 0.941200017929077
20 0.945900201797485
21 0.950800061225891
22 0.951099991798401
23 0.953999996185303
24 0.955499887466431
25 0.953299999237061
26 0.959100008010864
27 0.958900094032288
28 0.962400078773499
29 0.963500022888184
31 0.95990002155304
32 0.961100101470947
33 0.964600086212158
34 0.969799995422363
35 0.967200040817261
36 0.970999956130981
37 0.971100091934204
38 0.973600149154663
39 0.970099925994873
40 0.972700119018555
41 0.970800161361694
42 0.971400022506714
43 0.972599983215332
44 0.973000049591064
45 0.970499992370605
46 0.974900007247925
47 0.973600149154663
48 0.971199989318848
49 0.969099998474121
50 0.971800088882446
51 0.974200010299683
52 0.967800140380859
53 0.973900079727173
54 0.975100040435791
55 0.971499919891357
56 0.970299959182739
57 0.975900173187256
58 0.971500039100647
59 0.972700119018555
60 0.975200176239014
61 0.973099946975708
62 0.976400136947632
63 0.976300001144409
64 0.97350001335144
65 0.97730016708374
66 0.978300094604492
67 0.975399971008301
68 0.975200176239014
69 0.977900147438049
70 0.97760009765625
71 0.975300073623657
72 0.970900177955627
73 0.969099998474121
74 0.976100087165833
75 0.976900100708008
76 0.975500106811523
77 0.974499940872192
78 0.971199989318848
79 0.975300073623657
80 0.972800016403198
81 0.976600170135498
82 0.977400064468384
83 0.975500106811523
84 0.975600004196167
85 0.97379994392395
86 0.976200103759766
87 0.979000091552734
88 0.972900032997131
89 0.978200078010559
90 0.976900219917297
91 0.970900058746338
92 0.979200124740601
93 0.975600004196167
94 0.977400064468384
95 0.978600144386292
96 0.977699995040894
97 0.976000070571899
98 0.973000049591064
99 0.975899934768677
100 0.978399991989136
101 0.979300260543823
102 0.978900194168091
103 0.97979998588562
104 0.97819995880127
105 0.979000091552734
106 0.977500200271606
107 0.979400157928467
108 0.97950005531311
109 0.97730016708374
110 0.978700160980225
111 0.97950005531311
112 0.979000091552734
113 0.976500153541565
114 0.979700088500977
115 0.976700067520142
116 0.978800058364868
117 0.977200031280518
118 0.97760009765625
119 0.979900121688843
120 0.980700135231018
121 0.980500221252441
122 0.979800224304199
123 0.979700088500977
124 0.979099988937378
125 0.979400157928467
126 0.980900049209595
128 0.979400157928467
129 0.979700088500977
130 0.979099988937378
131 0.981199979782104
132 0.980700135231018
133 0.979900121688843
134 0.97950005531311
135 0.980100154876709
136 0.979000091552734
137 0.981400012969971
138 0.980200052261353
139 0.974200010299683
140 0.980000138282776
142 0.980499982833862
143 0.980700016021729
144 0.980499982833862
145 0.980700016021729
146 0.978900074958801
147 0.980600118637085
148 0.979700088500977
149 0.980700135231018
150 0.980900049209595
151 0.980800151824951
152 0.979300022125244
153 0.980300188064575
154 0.97979998588562
155 0.981000185012817
156 0.980700016021729
157 0.980700135231018
158 0.979900121688843
159 0.980100154876709
160 0.97950005531311
161 0.980500221252441
162 0.979800224304199
163 0.980300068855286
164 0.978900074958801
165 0.980100154876709
166 0.978700160980225
167 0.980300188064575
168 0.980400085449219
169 0.980800151824951
170 0.979099988937378
171 0.980200052261353
172 0.980000138282776
173 0.980900049209595
174 0.980700016021729
175 0.980800151824951
176 0.977400064468384
177 0.978800058364868
178 0.980900049209595
179 0.980900049209595
180 0.98110020160675
181 0.981000065803528
182 0.979399919509888
183 0.979900121688843
184 0.979900121688843
186 0.981000185012817
188 0.980000138282776
189 0.979900121688843
190 0.980900049209595
192 0.981200218200684
193 0.980900049209595
194 0.980100154876709
195 0.980700135231018
196 0.980500221252441
197 0.981100082397461
198 0.981100082397461
199 0.980900049209595
200 0.97950005531311
201 0.980200052261353
203 0.981100082397461
204 0.980700016021729
205 0.981000065803528
206 0.978600025177002
207 0.979700207710266
209 0.980999946594238
211 0.980800151824951
212 0.979200124740601
213 0.979700207710266
214 0.980400085449219
215 0.980800151824951
216 0.98140013217926
217 0.980800151824951
218 0.980900049209595
219 0.980100154876709
220 0.981100082397461
221 0.980700016021729
222 0.981199979782104
223 0.980600118637085
224 0.979700088500977
225 0.97979998588562
226 0.980800151824951
227 0.981100082397461
228 0.981100082397461
229 0.980300068855286
230 0.979700088500977
231 0.979700207710266
232 0.980400085449219
233 0.980900049209595
234 0.981100082397461
237 0.97950005531311
238 0.980300188064575
239 0.980800151824951
};
\addlegendentry{Tayla, p=1, H=6}
\addplot [line width=2pt, color1]
table {%
0 0.977299928665161
239 0.977299928665161
};
\addlegendentry{RNODE}
\addplot [line width=2pt, color2]
table {%
0 0.978900194168091
239 0.978900194168091
};
\addlegendentry{TayNode}
\addplot [line width=2pt, white!50.1960784313725!black]
table {%
0 0.979099988937378
239 0.979099988937378
};
\addlegendentry{Vanilla NeuralODE}
\end{axis}

\end{tikzpicture}


==> figs/mnist/predaccuracy_data.tex <==
\definecolor{color0}{rgb}{1,1,0}
\definecolor{color1}{rgb}{1,0,1}
\definecolor{color2}{rgb}{0,1,1}

\addplot [thick, blue]
table {%
0 0.658100008964539
1 0.803100109100342
2 0.867100238800049
3 0.89109992980957
4 0.905400276184082
5 0.90690016746521
6 0.911800026893616
7 0.909000158309937
8 0.919400215148926
9 0.921299934387207
10 0.92300009727478
11 0.918200135231018
12 0.928200006484985
13 0.92710018157959
14 0.932699918746948
15 0.936100125312805
16 0.942000150680542
17 0.940600156784058
18 0.945800065994263
19 0.939600110054016
20 0.947600126266479
21 0.954600095748901
22 0.951900005340576
23 0.951500177383423
24 0.956799983978271
25 0.954200029373169
26 0.959700107574463
27 0.956100106239319
28 0.959500074386597
29 0.965200066566467
30 0.964999914169312
31 0.957300186157227
32 0.964300155639648
33 0.966400146484375
34 0.963100075721741
35 0.960400104522705
36 0.96969997882843
37 0.968600034713745
38 0.968800067901611
39 0.972300171852112
40 0.970800042152405
41 0.968699932098389
42 0.969800114631653
43 0.970500111579895
44 0.970800042152405
45 0.967700004577637
46 0.972100019454956
47 0.972000122070312
48 0.972400188446045
49 0.969600200653076
50 0.969099998474121
51 0.970700025558472
52 0.969799995422363
53 0.969599962234497
54 0.973800182342529
55 0.974800109863281
56 0.970900058746338
57 0.976000070571899
58 0.972100019454956
59 0.970700025558472
60 0.975000143051147
61 0.974000215530396
62 0.97160005569458
63 0.976100206375122
64 0.97760009765625
65 0.971500039100647
66 0.976000070571899
67 0.974400043487549
68 0.973200082778931
69 0.977200150489807
70 0.975800037384033
71 0.973600029945374
72 0.976599931716919
73 0.975500106811523
74 0.975300073623657
75 0.978100061416626
76 0.977800130844116
77 0.973800182342529
78 0.978500127792358
79 0.971400022506714
80 0.973200082778931
81 0.975399971008301
82 0.978800296783447
83 0.976500153541565
84 0.975800156593323
85 0.974400162696838
86 0.974100112915039
87 0.97979998588562
88 0.979900121688843
89 0.977699995040894
90 0.979200005531311
91 0.97790002822876
92 0.972599983215332
93 0.974700093269348
94 0.977200150489807
95 0.978100061416626
96 0.976200103759766
97 0.975800156593323
98 0.976999998092651
99 0.976800084114075
100 0.978800058364868
101 0.979700088500977
102 0.978100061416626
104 0.980100154876709
105 0.980599999427795
106 0.976500034332275
107 0.980400085449219
108 0.979900002479553
109 0.979099988937378
110 0.976900100708008
111 0.979700088500977
112 0.976999998092651
113 0.980500221252441
114 0.977800130844116
115 0.978100061416626
116 0.979200005531311
117 0.981500148773193
118 0.977200031280518
119 0.980400204658508
120 0.981800079345703
121 0.982399940490723
122 0.977500081062317
123 0.981200218200684
124 0.981800079345703
125 0.981100082397461
126 0.98229992389679
127 0.981500148773193
128 0.980900049209595
129 0.982000112533569
130 0.980200052261353
131 0.981900215148926
132 0.980600118637085
133 0.982600212097168
134 0.980800151824951
135 0.981000065803528
136 0.980599999427795
137 0.982300043106079
138 0.982400059700012
139 0.980700016021729
140 0.981800079345703
141 0.981600046157837
142 0.98229992389679
143 0.982500195503235
144 0.982899904251099
145 0.982000112533569
146 0.981400012969971
147 0.981100082397461
148 0.983200073242188
150 0.981899976730347
152 0.982300043106079
153 0.98170018196106
154 0.982500076293945
155 0.981899976730347
156 0.982100129127502
158 0.981899976730347
159 0.981000065803528
160 0.981199979782104
161 0.980499982833862
162 0.983200073242188
163 0.981600046157837
165 0.981400012969971
166 0.982500076293945
167 0.98170006275177
168 0.982700109481812
169 0.982599973678589
170 0.979900121688843
171 0.982100009918213
173 0.982100009918213
174 0.979600071907043
175 0.982500076293945
176 0.982300043106079
177 0.98170006275177
178 0.983000040054321
179 0.981899976730347
180 0.982699990272522
181 0.982199907302856
182 0.983200073242188
183 0.981600046157837
184 0.981800079345703
185 0.982800006866455
186 0.982400059700012
187 0.983100056648254
188 0.98170018196106
189 0.981600046157837
190 0.98170006275177
191 0.981199979782104
193 0.982699990272522
194 0.980200052261353
195 0.982100009918213
196 0.982200145721436
197 0.981800079345703
198 0.983700037002563
199 0.981100082397461
200 0.983000040054321
201 0.982200145721436
202 0.982100009918213
203 0.981600046157837
204 0.982200145721436
205 0.983100056648254
206 0.982700109481812
207 0.981300115585327
208 0.982300043106079
209 0.981800079345703
210 0.982800126075745
211 0.982500076293945
212 0.982400059700012
213 0.981100082397461
214 0.979100227355957
215 0.982900142669678
216 0.982400178909302
219 0.982300043106079
220 0.978900074958801
221 0.98170006275177
222 0.982800006866455
223 0.982700109481812
224 0.982100009918213
225 0.982400059700012
226 0.981899976730347
227 0.981600046157837
228 0.983100056648254
229 0.983500123023987
230 0.982800006866455
231 0.982300043106079
232 0.982700109481812
233 0.98199999332428
234 0.98330020904541
235 0.983000040054321
236 0.983200073242188
237 0.982500076293945
238 0.978800058364868
239 0.982900142669678
};
% \addlegendentry{Tayla, p=2, H=2}
\addplot [thick, green!50.1960784313725!black]
table {%
0 0.662699937820435
1 0.778600096702576
2 0.815700054168701
3 0.862900018692017
4 0.885699987411499
5 0.898200035095215
6 0.902200222015381
7 0.908099889755249
8 0.91349995136261
9 0.913400173187256
10 0.916800022125244
11 0.914799928665161
12 0.919800043106079
13 0.922100067138672
14 0.923400044441223
15 0.926700115203857
16 0.928499937057495
17 0.930800080299377
18 0.932000160217285
19 0.930999994277954
20 0.934900045394897
21 0.942600011825562
22 0.940000057220459
23 0.946500062942505
24 0.944400072097778
25 0.945500135421753
26 0.952100038528442
27 0.955300092697144
28 0.954400062561035
29 0.959200024604797
30 0.956500053405762
31 0.958400249481201
32 0.959200024604797
33 0.958700180053711
34 0.964900016784668
35 0.953200101852417
36 0.963299989700317
37 0.960400104522705
38 0.964800000190735
39 0.967600107192993
40 0.96779990196228
41 0.966500043869019
43 0.964400053024292
44 0.967400074005127
45 0.964100003242493
46 0.966300249099731
47 0.967900037765503
48 0.964299917221069
49 0.964699983596802
50 0.966399908065796
51 0.970299959182739
52 0.971699953079224
53 0.967900037765503
54 0.970599889755249
55 0.968400120735168
56 0.968199968338013
57 0.972300171852112
58 0.97379994392395
59 0.964400053024292
60 0.972100019454956
61 0.972000122070312
62 0.970400094985962
64 0.971400022506714
65 0.968900203704834
66 0.970500111579895
67 0.967200040817261
68 0.973900079727173
69 0.975100040435791
70 0.969300031661987
71 0.974700212478638
72 0.968600034713745
73 0.968800187110901
74 0.972100257873535
75 0.976000070571899
76 0.972399950027466
77 0.969000101089478
78 0.974200010299683
79 0.973600149154663
80 0.972500085830688
81 0.974600076675415
82 0.974499940872192
83 0.971100091934204
84 0.97540009021759
85 0.968400239944458
86 0.97570013999939
87 0.970999956130981
88 0.970700025558472
89 0.975899934768677
90 0.973000049591064
91 0.970300197601318
92 0.971900105476379
93 0.974999904632568
94 0.97350001335144
95 0.969500064849854
96 0.966799974441528
97 0.975500106811523
98 0.973100185394287
99 0.97350025177002
100 0.977500081062317
101 0.977500081062317
102 0.975600004196167
103 0.976900100708008
104 0.976600170135498
105 0.97790002822876
106 0.976500034332275
107 0.976999998092651
108 0.974000096321106
109 0.976900100708008
110 0.975900173187256
111 0.978400230407715
112 0.97790002822876
113 0.976900100708008
114 0.975600004196167
115 0.975800037384033
116 0.977999925613403
117 0.978700160980225
119 0.974800109863281
120 0.977800011634827
121 0.977200031280518
122 0.977200031280518
123 0.976700067520142
124 0.976999998092651
125 0.977699995040894
126 0.979099988937378
127 0.976500034332275
128 0.978300094604492
129 0.976999998092651
130 0.976999998092651
131 0.974699974060059
132 0.979399919509888
133 0.977699995040894
134 0.975100040435791
135 0.97760009765625
136 0.977099895477295
137 0.976099967956543
138 0.976500034332275
139 0.977800130844116
140 0.978500127792358
141 0.97760009765625
142 0.97700023651123
143 0.977499961853027
144 0.978500008583069
145 0.976400375366211
146 0.978200078010559
147 0.978000164031982
149 0.976700067520142
150 0.978100061416626
151 0.977800130844116
152 0.978800058364868
153 0.97790002822876
154 0.977800130844116
155 0.976700067520142
156 0.977499961853027
157 0.976900100708008
158 0.978400230407715
159 0.978300094604492
160 0.977299928665161
161 0.976800084114075
162 0.978200197219849
163 0.978900074958801
164 0.978800058364868
165 0.978100061416626
166 0.97790002822876
167 0.976400017738342
168 0.978900194168091
169 0.97790002822876
170 0.978399991989136
172 0.977800130844116
173 0.978100061416626
174 0.978700160980225
175 0.978000164031982
176 0.978500127792358
177 0.978200078010559
178 0.978300094604492
179 0.977900147438049
180 0.978900194168091
181 0.979300141334534
182 0.979000091552734
183 0.977299928665161
184 0.97790002822876
185 0.977299928665161
186 0.978100061416626
188 0.979000091552734
189 0.978700160980225
190 0.977499961853027
191 0.977699995040894
192 0.978800058364868
193 0.977100133895874
194 0.978899955749512
195 0.978000164031982
196 0.977500081062317
197 0.97730016708374
198 0.979200124740601
199 0.979800224304199
200 0.978800058364868
201 0.978000164031982
202 0.978500008583069
203 0.97790002822876
204 0.978900194168091
205 0.979000091552734
207 0.97790002822876
208 0.977100014686584
209 0.97760009765625
210 0.979200124740601
211 0.978400230407715
212 0.978600144386292
213 0.978200078010559
214 0.97760009765625
215 0.978899955749512
216 0.978700160980225
217 0.980000019073486
218 0.978100061416626
219 0.978600025177002
220 0.977299928665161
221 0.977400064468384
223 0.979099988937378
224 0.978800058364868
225 0.978300094604492
226 0.978600144386292
227 0.976699948310852
228 0.979400157928467
229 0.979099988937378
230 0.979200124740601
231 0.979000091552734
232 0.978200078010559
233 0.976399898529053
235 0.979900121688843
236 0.979400157928467
237 0.978500127792358
238 0.978700160980225
239 0.977200031280518
};
% \addlegendentry{Tayla, p=1, H=2}
\addplot [thick, color0]
table {%
0 0.667799949645996
1 0.801800012588501
2 0.857600212097168
3 0.888700127601624
4 0.899900078773499
5 0.907000064849854
6 0.914499998092651
7 0.910700082778931
8 0.917700052261353
9 0.917900085449219
10 0.921600103378296
11 0.922199964523315
12 0.926300168037415
14 0.93120002746582
15 0.928300142288208
16 0.936599969863892
17 0.938600182533264
18 0.942999958992004
19 0.941200017929077
20 0.945900201797485
21 0.950800061225891
22 0.951099991798401
23 0.953999996185303
24 0.955499887466431
25 0.953299999237061
26 0.959100008010864
27 0.958900094032288
28 0.962400078773499
29 0.963500022888184
31 0.95990002155304
32 0.961100101470947
33 0.964600086212158
34 0.969799995422363
35 0.967200040817261
36 0.970999956130981
37 0.971100091934204
38 0.973600149154663
39 0.970099925994873
40 0.972700119018555
41 0.970800161361694
42 0.971400022506714
43 0.972599983215332
44 0.973000049591064
45 0.970499992370605
46 0.974900007247925
47 0.973600149154663
48 0.971199989318848
49 0.969099998474121
50 0.971800088882446
51 0.974200010299683
52 0.967800140380859
53 0.973900079727173
54 0.975100040435791
55 0.971499919891357
56 0.970299959182739
57 0.975900173187256
58 0.971500039100647
59 0.972700119018555
60 0.975200176239014
61 0.973099946975708
62 0.976400136947632
63 0.976300001144409
64 0.97350001335144
65 0.97730016708374
66 0.978300094604492
67 0.975399971008301
68 0.975200176239014
69 0.977900147438049
70 0.97760009765625
71 0.975300073623657
72 0.970900177955627
73 0.969099998474121
74 0.976100087165833
75 0.976900100708008
76 0.975500106811523
77 0.974499940872192
78 0.971199989318848
79 0.975300073623657
80 0.972800016403198
81 0.976600170135498
82 0.977400064468384
83 0.975500106811523
84 0.975600004196167
85 0.97379994392395
86 0.976200103759766
87 0.979000091552734
88 0.972900032997131
89 0.978200078010559
90 0.976900219917297
91 0.970900058746338
92 0.979200124740601
93 0.975600004196167
94 0.977400064468384
95 0.978600144386292
96 0.977699995040894
97 0.976000070571899
98 0.973000049591064
99 0.975899934768677
100 0.978399991989136
101 0.979300260543823
102 0.978900194168091
103 0.97979998588562
104 0.97819995880127
105 0.979000091552734
106 0.977500200271606
107 0.979400157928467
108 0.97950005531311
109 0.97730016708374
110 0.978700160980225
111 0.97950005531311
112 0.979000091552734
113 0.976500153541565
114 0.979700088500977
115 0.976700067520142
116 0.978800058364868
117 0.977200031280518
118 0.97760009765625
119 0.979900121688843
120 0.980700135231018
121 0.980500221252441
122 0.979800224304199
123 0.979700088500977
124 0.979099988937378
125 0.979400157928467
126 0.980900049209595
128 0.979400157928467
129 0.979700088500977
130 0.979099988937378
131 0.981199979782104
132 0.980700135231018
133 0.979900121688843
134 0.97950005531311
135 0.980100154876709
136 0.979000091552734
137 0.981400012969971
138 0.980200052261353
139 0.974200010299683
140 0.980000138282776
142 0.980499982833862
143 0.980700016021729
144 0.980499982833862
145 0.980700016021729
146 0.978900074958801
147 0.980600118637085
148 0.979700088500977
149 0.980700135231018
150 0.980900049209595
151 0.980800151824951
152 0.979300022125244
153 0.980300188064575
154 0.97979998588562
155 0.981000185012817
156 0.980700016021729
157 0.980700135231018
158 0.979900121688843
159 0.980100154876709
160 0.97950005531311
161 0.980500221252441
162 0.979800224304199
163 0.980300068855286
164 0.978900074958801
165 0.980100154876709
166 0.978700160980225
167 0.980300188064575
168 0.980400085449219
169 0.980800151824951
170 0.979099988937378
171 0.980200052261353
172 0.980000138282776
173 0.980900049209595
174 0.980700016021729
175 0.980800151824951
176 0.977400064468384
177 0.978800058364868
178 0.980900049209595
179 0.980900049209595
180 0.98110020160675
181 0.981000065803528
182 0.979399919509888
183 0.979900121688843
184 0.979900121688843
186 0.981000185012817
188 0.980000138282776
189 0.979900121688843
190 0.980900049209595
192 0.981200218200684
193 0.980900049209595
194 0.980100154876709
195 0.980700135231018
196 0.980500221252441
197 0.981100082397461
198 0.981100082397461
199 0.980900049209595
200 0.97950005531311
201 0.980200052261353
203 0.981100082397461
204 0.980700016021729
205 0.981000065803528
206 0.978600025177002
207 0.979700207710266
209 0.980999946594238
211 0.980800151824951
212 0.979200124740601
213 0.979700207710266
214 0.980400085449219
215 0.980800151824951
216 0.98140013217926
217 0.980800151824951
218 0.980900049209595
219 0.980100154876709
220 0.981100082397461
221 0.980700016021729
222 0.981199979782104
223 0.980600118637085
224 0.979700088500977
225 0.97979998588562
226 0.980800151824951
227 0.981100082397461
228 0.981100082397461
229 0.980300068855286
230 0.979700088500977
231 0.979700207710266
232 0.980400085449219
233 0.980900049209595
234 0.981100082397461
237 0.97950005531311
238 0.980300188064575
239 0.980800151824951
};
% \addlegendentry{Tayla, p=1, H=6}
\addplot [ultra thick, color1]
table {%
0 0.977299928665161
239 0.977299928665161
};
% \addlegendentry{RNODE}
\addplot [ultra thick, black, dashed]
table {%
0 0.978900194168091
239 0.978900194168091
};
% \addlegendentry{TayNode}
\addplot [ultra thick, white!50.1960784313725!black]
table {%
0 0.979099988937378
239 0.979099988937378
};
% \addlegendentry{Vanilla NeuralODE}

==> figs/stiff_dynamics/accuracy_dt_data.tex <==
% \path [fill=blue, fill opacity=0.6, ultra thick]
% (axis cs:0.001,0.00674892068804359)
% --(axis cs:0.001,0.00628083985872814)
% --(axis cs:0.005,0.968643031291001)
% --(axis cs:0.01,0.998528384736213)
% --(axis cs:0.05,0.999998289853123)
% --(axis cs:0.1,0.999999902196237)
% --(axis cs:0.15,0.999999981862288)
% --(axis cs:0.2,0.999999994576851)
% --(axis cs:0.25,0.999999997895373)
% --(axis cs:0.3,0.999999999037089)
% --(axis cs:0.3,0.999999999172195)
% --(axis cs:0.3,0.999999999172195)
% --(axis cs:0.25,0.999999998190672)
% --(axis cs:0.2,0.999999995337771)
% --(axis cs:0.15,0.99999998440718)
% --(axis cs:0.1,0.99999991591903)
% --(axis cs:0.05,0.999998529802695)
% --(axis cs:0.01,0.998734678046545)
% --(axis cs:0.005,0.972889832413141)
% --(axis cs:0.001,0.00674892068804359)
% --cycle;

% \path [fill=color0, fill opacity=0.6, ultra thick]
% (axis cs:0.001,0.114005861635813)
% --(axis cs:0.001,0.107168306162876)
% --(axis cs:0.005,0.950040447874012)
% --(axis cs:0.01,0.98961347968663)
% --(axis cs:0.05,0.999657211542497)
% --(axis cs:0.1,0.9999200826597)
% --(axis cs:0.15,0.999966436946817)
% --(axis cs:0.2,0.999982101115632)
% --(axis cs:0.25,0.999989125117729)
% --(axis cs:0.3,0.999992825868898)
% --(axis cs:0.3,0.999993832463533)
% --(axis cs:0.3,0.999993832463533)
% --(axis cs:0.25,0.999990650957752)
% --(axis cs:0.2,0.999984612474409)
% --(axis cs:0.15,0.999971146076017)
% --(axis cs:0.1,0.999931295337842)
% --(axis cs:0.05,0.99970529915412)
% --(axis cs:0.01,0.991062450400552)
% --(axis cs:0.005,0.956734044314968)
% --(axis cs:0.001,0.114005861635813)
% --cycle;

% \path [fill=green!50.1960784313725!black, fill opacity=0.6, ultra thick]
% (axis cs:0.001,0.00248060726312943)
% --(axis cs:0.001,0.00228415011222909)
% --(axis cs:0.005,0.000950362577960685)
% --(axis cs:0.01,0.00409396416070698)
% --(axis cs:0.05,0.289368284497558)
% --(axis cs:0.1,0.709352658117715)
% --(axis cs:0.15,0.809589911254479)
% --(axis cs:0.2,0.620555751992536)
% --(axis cs:0.25,0.973855702687465)
% --(axis cs:0.3,0.868234067939382)
% --(axis cs:0.3,0.919165507623551)
% --(axis cs:0.3,0.919165507623551)
% --(axis cs:0.25,0.978279052731022)
% --(axis cs:0.2,0.682107753579968)
% --(axis cs:0.15,0.822961671082601)
% --(axis cs:0.1,0.738913595800321)
% --(axis cs:0.05,0.35861034005146)
% --(axis cs:0.01,0.00466207977715654)
% --(axis cs:0.005,0.00112661887661256)
% --(axis cs:0.001,0.00248060726312943)
% --cycle;

% \path [fill=color1, fill opacity=0.6, ultra thick]
% (axis cs:0.001,1.30394672883838e-09)
% --(axis cs:0.001,1.21189339323927e-09)
% --(axis cs:0.005,6.91797422526507e-09)
% --(axis cs:0.01,7.06417986379943e-08)
% --(axis cs:0.05,1.14004457840293e-05)
% --(axis cs:0.1,9.67137276414096e-05)
% --(axis cs:0.15,0.000341917131129647)
% --(axis cs:0.2,0.000845291889666812)
% --(axis cs:0.25,0.00171839254478716)
% --(axis cs:0.3,0.00308533563887487)
% --(axis cs:0.3,0.00308598455419381)
% --(axis cs:0.3,0.00308598455419381)
% --(axis cs:0.25,0.0017188643150621)
% --(axis cs:0.2,0.000845529416688726)
% --(axis cs:0.15,0.00034202724961325)
% --(axis cs:0.1,9.67608471847376e-05)
% --(axis cs:0.05,1.14221735858279e-05)
% --(axis cs:0.01,7.0747622807106e-08)
% --(axis cs:0.005,6.92948897421526e-09)
% --(axis cs:0.001,1.30394672883838e-09)
% --cycle;

% \path [fill=color2, fill opacity=0.6, ultra thick]
% (axis cs:0.001,4.99625240714309e-13)
% --(axis cs:0.001,4.6484000290608e-13)
% --(axis cs:0.005,1.71345925138905e-10)
% --(axis cs:0.01,3.68303590047446e-10)
% --(axis cs:0.05,1.34237127173002e-07)
% --(axis cs:0.1,2.44637961223252e-06)
% --(axis cs:0.15,1.28384602520267e-05)
% --(axis cs:0.2,4.24763953149032e-05)
% --(axis cs:0.25,0.000107468420937031)
% --(axis cs:0.3,0.000232621421562565)
% --(axis cs:0.3,0.0002328751118447)
% --(axis cs:0.3,0.0002328751118447)
% --(axis cs:0.25,0.000107582716663363)
% --(axis cs:0.2,4.24838576019708e-05)
% --(axis cs:0.15,1.28430029207768e-05)
% --(axis cs:0.1,2.45447886717472e-06)
% --(axis cs:0.05,1.34810744852659e-07)
% --(axis cs:0.01,4.09063893143655e-10)
% --(axis cs:0.005,2.00050300491404e-10)
% --(axis cs:0.001,4.99625240714309e-13)
% --cycle;

% \path [fill=white!50.1960784313725!black, fill opacity=0.6, ultra thick]
% (axis cs:0.001,3.27714725986535e-13)
% --(axis cs:0.001,3.04764258168238e-13)
% --(axis cs:0.005,4.25149856208341e-14)
% --(axis cs:0.01,4.09054963975817e-13)
% --(axis cs:0.05,2.74926188604018e-15)
% --(axis cs:0.1,3.45795271968738e-13)
% --(axis cs:0.15,1.80799980551745e-12)
% --(axis cs:0.2,2.1044762084956e-13)
% --(axis cs:0.25,2.71771285385582e-14)
% --(axis cs:0.3,1.01487725519647e-12)
% --(axis cs:0.3,1.1824407184687e-12)
% --(axis cs:0.3,1.1824407184687e-12)
% --(axis cs:0.25,3.15941100578055e-14)
% --(axis cs:0.2,2.45166675594389e-13)
% --(axis cs:0.15,2.10645713444609e-12)
% --(axis cs:0.1,4.02860148483566e-13)
% --(axis cs:0.05,3.21540883343834e-15)
% --(axis cs:0.01,4.76541608564852e-13)
% --(axis cs:0.005,4.95011543602107e-14)
% --(axis cs:0.001,3.27714725986535e-13)
% --cycle;

\addplot [ultra thick, blue, mark=asterisk, mark size=3, mark options={solid}]
table {%
0.0010000467300415 0.00651488034054637
0.00499999523162842 0.970766484737396
0.00999999046325684 0.998631536960602
0.0499999523162842 0.999998331069946
0.100000023841858 1
0.149999976158142 1
0.200000047683716 1
0.25 1
0.299999952316284 1
};
% \addlegendentry{RK4}
\addplot [ultra thick, color0, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0010000467300415 0.110587082803249
0.00499999523162842 0.953387379646301
0.00999999046325684 0.990338027477264
0.0499999523162842 0.999681353569031
0.100000023841858 0.99992561340332
0.149999976158142 0.999968707561493
0.200000047683716 0.999983251094818
0.25 0.999989867210388
0.299999952316284 0.99999338388443
};
% \addlegendentry{Taylor, o=2}
\addplot [ultra thick, green!50.1960784313725!black, mark=+, mark size=3, mark options={solid}]
table {%
0.0010000467300415 0.00238237879239023
0.00499999523162842 0.00103849091101438
0.00999999046325684 0.00437802309170365
0.0499999523162842 0.32398933172226
0.100000023841858 0.724133193492889
0.149999976158142 0.816275715827942
0.200000047683716 0.651331722736359
0.25 0.976067364215851
0.299999952316284 0.893699824810028
};
% \addlegendentry{Hyper, o=1}
\addplot [ultra thick, color1, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.0010000467300415 1.25792065652774e-09
0.00499999523162842 6.92373802735347e-09
0.00999999046325684 7.06946750028692e-08
0.0499999523162842 1.14113063318655e-05
0.100000023841858 9.67372616287321e-05
0.149999976158142 0.000341972248861566
0.200000047683716 0.000845410744659603
0.25 0.00171862868592143
0.299999952316284 0.00308566074818373
};
% \addlegendentry{Tayla, o=1}
\addplot [ultra thick, color2, mark=square*, mark size=3, mark options={solid}]
table {%
0.0010000467300415 4.82232147009515e-13
0.00499999523162842 1.8569808191149e-10
0.00999999046325684 3.88684084917656e-10
0.0499999523162842 1.34523901351713e-07
0.100000023841858 2.45042929236661e-06
0.149999976158142 1.28407282318221e-05
0.200000047683716 4.24801219196524e-05
0.25 0.000107525578641798
0.299999952316284 0.000232748221606016
};
% \addlegendentry{Tayla, o=2}
\addplot [ultra thick, white!50.1960784313725!black, mark=*, mark size=3, mark options={solid, fill=white!50.1960784313725!black}]
table {%
0.0010000467300415 3.1623957467454e-13
0.00499999523162842 4.60080853081045e-14
0.00999999046325684 4.42798250323284e-13
0.0499999523162842 2.98233842102016e-15
0.100000023841858 3.74327494999036e-13
0.149999976158142 1.95722713210167e-12
0.200000047683716 2.27807383417281e-13
0.25 2.9385622759984e-14
0.299999952316284 1.09865924951408e-12
};
% \addlegendentry{Dopri5}

==> figs/stiff_dynamics/cTime_dt_data.tex <==
\path [fill=blue, fill opacity=0.6, thick]
(axis cs:0.001,4.4877881476962e-05)
--(axis cs:0.001,3.30845160965052e-05)
--(axis cs:0.005,2.9440905999989e-05)
--(axis cs:0.01,3.55271522681186e-05)
--(axis cs:0.05,3.4332275390625e-05)
--(axis cs:0.1,3.61006247414927e-05)
--(axis cs:0.15,3.33786010742188e-05)
--(axis cs:0.2,3.48145367622256e-05)
--(axis cs:0.25,3.31401824951172e-05)
--(axis cs:0.3,3.4332275390625e-05)
--(axis cs:0.3,4.05311584472656e-05)
--(axis cs:0.3,4.05311584472656e-05)
--(axis cs:0.25,4.08391046666142e-05)
--(axis cs:0.2,4.0048897075665e-05)
--(axis cs:0.15,3.97554547957456e-05)
--(axis cs:0.1,4.11469948874136e-05)
--(axis cs:0.05,4.66612495160372e-05)
--(axis cs:0.01,5.67294845785146e-05)
--(axis cs:0.005,3.51857813035476e-05)
--(axis cs:0.001,4.4877881476962e-05)
--cycle;

\path [fill=color0, fill opacity=0.6, thick]
(axis cs:0.001,2.98980381426504e-05)
--(axis cs:0.001,2.63607833129235e-05)
--(axis cs:0.005,2.38418579101562e-05)
--(axis cs:0.01,2.74181365966797e-05)
--(axis cs:0.05,3.47484949589244e-05)
--(axis cs:0.1,2.6702880859375e-05)
--(axis cs:0.15,2.75655066306877e-05)
--(axis cs:0.2,2.74181365966797e-05)
--(axis cs:0.25,2.76565551757812e-05)
--(axis cs:0.3,2.86102294921875e-05)
--(axis cs:0.3,3.09944152832031e-05)
--(axis cs:0.3,3.09944152832031e-05)
--(axis cs:0.25,3.20041497698478e-05)
--(axis cs:0.2,3.127906641573e-05)
--(axis cs:0.15,4.08946853684752e-05)
--(axis cs:0.1,2.97405229240053e-05)
--(axis cs:0.05,4.20576087827568e-05)
--(axis cs:0.01,4.47285050586712e-05)
--(axis cs:0.005,3.34161467341768e-05)
--(axis cs:0.001,2.98980381426504e-05)
--cycle;

\path [fill=green!50.1960784313725!black, fill opacity=0.6, thick]
(axis cs:0.001,7.14927827865606e-05)
--(axis cs:0.001,5.12687365493117e-05)
--(axis cs:0.005,5.31673431396484e-05)
--(axis cs:0.01,5.70786851176277e-05)
--(axis cs:0.05,5.74588775634766e-05)
--(axis cs:0.1,6.03199005126953e-05)
--(axis cs:0.15,6.56540853261626e-05)
--(axis cs:0.2,5.98051574465818e-05)
--(axis cs:0.25,5.86509704589844e-05)
--(axis cs:0.3,6.22272491455078e-05)
--(axis cs:0.3,6.96182250976562e-05)
--(axis cs:0.3,6.96182250976562e-05)
--(axis cs:0.25,6.42397952324003e-05)
--(axis cs:0.2,6.58414337399416e-05)
--(axis cs:0.15,8.81599579913598e-05)
--(axis cs:0.1,6.7720123163348e-05)
--(axis cs:0.05,7.05646186900059e-05)
--(axis cs:0.01,6.87576677951195e-05)
--(axis cs:0.005,0.000123959526561154)
--(axis cs:0.001,7.14927827865606e-05)
--cycle;

\path [fill=color1, fill opacity=0.6, thick]
(axis cs:0.001,4.04450826619765e-05)
--(axis cs:0.001,3.37137661432185e-05)
--(axis cs:0.005,3.26633453369141e-05)
--(axis cs:0.01,3.44010617460614e-05)
--(axis cs:0.05,3.55405773569831e-05)
--(axis cs:0.1,3.91006469726562e-05)
--(axis cs:0.15,3.74317169189453e-05)
--(axis cs:0.2,3.91006469726562e-05)
--(axis cs:0.25,3.88622283935547e-05)
--(axis cs:0.3,4.02927398681641e-05)
--(axis cs:0.3,4.81605529785156e-05)
--(axis cs:0.3,4.81605529785156e-05)
--(axis cs:0.25,4.48346851683285e-05)
--(axis cs:0.2,4.54511865449494e-05)
--(axis cs:0.15,4.23103659069406e-05)
--(axis cs:0.1,4.43724091440924e-05)
--(axis cs:0.05,4.08063498619839e-05)
--(axis cs:0.01,4.23145762913801e-05)
--(axis cs:0.005,4.09734395874358e-05)
--(axis cs:0.001,4.04450826619765e-05)
--cycle;

\path [fill=color2, fill opacity=0.6, thick]
(axis cs:0.001,6.02666594749954e-05)
--(axis cs:0.001,4.30372281668247e-05)
--(axis cs:0.005,4.36305999755859e-05)
--(axis cs:0.01,4.45842742919922e-05)
--(axis cs:0.05,5.07831573486328e-05)
--(axis cs:0.1,4.92310533515938e-05)
--(axis cs:0.15,5.59833078373907e-05)
--(axis cs:0.2,5.29289245605469e-05)
--(axis cs:0.25,5.65348134837175e-05)
--(axis cs:0.3,5.22136688232422e-05)
--(axis cs:0.3,6.12735748291016e-05)
--(axis cs:0.3,6.12735748291016e-05)
--(axis cs:0.25,5.96046447753906e-05)
--(axis cs:0.2,6.18333999693324e-05)
--(axis cs:0.15,6.17954702387812e-05)
--(axis cs:0.1,5.51962842948906e-05)
--(axis cs:0.05,5.81507042827305e-05)
--(axis cs:0.01,5.18206150915908e-05)
--(axis cs:0.005,5.95139542250517e-05)
--(axis cs:0.001,6.02666594749954e-05)
--cycle;

\path [fill=white!50.1960784313725!black, fill opacity=0.6, thick]
(axis cs:0.001,0.000209152307093751)
--(axis cs:0.001,7.62939453125e-05)
--(axis cs:0.005,0.000106096267700195)
--(axis cs:0.01,0.000232934951782227)
--(axis cs:0.05,0.000853776931762695)
--(axis cs:0.1,0.00171138804917395)
--(axis cs:0.15,0.00218371626644763)
--(axis cs:0.2,0.00324395447863462)
--(axis cs:0.25,0.00397751824781511)
--(axis cs:0.3,0.00476908683776855)
--(axis cs:0.3,0.00479245185852051)
--(axis cs:0.3,0.00479245185852051)
--(axis cs:0.25,0.00418498022630599)
--(axis cs:0.2,0.00332566946850894)
--(axis cs:0.15,0.00226170032029205)
--(axis cs:0.1,0.00180596151188156)
--(axis cs:0.05,0.00115658198053448)
--(axis cs:0.01,0.000389035279528914)
--(axis cs:0.005,0.000384340194216811)
--(axis cs:0.001,0.000209152307093751)
--cycle;

\addplot [ultra thick, green!50.1960784313725!black, mark=+, mark size=3, mark options={solid}]
table {%
0.0010000467300415 6.13807278568856e-05
0.00499999523162842 8.57062477734871e-05
0.00999999046325684 6.29181813565083e-05
0.0499999523162842 6.35694450465962e-05
0.100000023841858 6.3916013459675e-05
0.149999976158142 7.69069883972406e-05
0.200000047683716 6.28232664894313e-05
0.25 6.10351708019152e-05
0.299999952316284 6.59227080177516e-05
};
\addlegendentry{Hypersolver}%, \(p=1\)}

\addplot [ultra thick, color0, mark=triangle*, mark size=3, mark options={solid}]
table {%
0.0010000467300415 2.81294069282012e-05
0.00499999523162842 2.85869409708539e-05
0.00999999046325684 3.55470583599526e-05
0.0499999523162842 3.84030608984176e-05
0.100000023841858 2.82128585240571e-05
0.149999976158142 3.42300954798702e-05
0.200000047683716 2.90274638246046e-05
0.25 2.97228634735802e-05
0.299999952316284 2.98023369396105e-05
};
\addlegendentry{Taylor, \(p=1\)}

\addplot [ultra thick, blue, mark=asterisk, mark size=3, mark options={solid}]
table {%
0.0010000467300415 3.89811939385254e-05
0.00499999523162842 3.23133353958838e-05
0.00999999046325684 4.61283161712345e-05
0.0499999523162842 3.96658106183168e-05
0.100000023841858 3.86237952625379e-05
0.149999976158142 3.62736936949659e-05
0.200000047683716 3.74317205569241e-05
0.25 3.63985673175193e-05
0.299999952316284 3.74317205569241e-05
};
\addlegendentry{RK4}

\addplot [ultra thick, color1, mark=diamond*, mark size=3, mark options={solid}]
table {%
0.0010000467300415 3.70794077753089e-05
0.00499999523162842 3.65831874660216e-05
0.00999999046325684 3.83578044420574e-05
0.0499999523162842 3.81734462280292e-05
0.100000023841858 4.15643044107128e-05
0.149999976158142 3.94412454625126e-05
0.200000047683716 4.22597076976672e-05
0.25 4.14053429267369e-05
0.299999952316284 4.42266209574882e-05
};
\addlegendentry{TL (ours), \(p=1\)}
\addplot [ultra thick, color2, mark=square*, mark size=3, mark options={solid}]
table {%
0.0010000467300415 5.16519357915968e-05
0.00499999523162842 5.13876584591344e-05
0.00999999046325684 4.80275484733284e-05
0.0499999523162842 5.336163303582e-05
0.100000023841858 5.2213690651115e-05
0.149999976158142 5.888940722798e-05
0.200000047683716 5.7339682825841e-05
0.25 5.83330802328419e-05
0.299999952316284 5.67436436540447e-05
};
\addlegendentry{TL (ours), \(p=2\)}
\addplot [ultra thick, white!50.1960784313725!black, mark=*, mark size=3, mark options={solid}]
table {%
0.0010000467300415 0.0001054843669408
0.00499999523162842 0.000164658151334152
0.00999999046325684 0.000259354012086987
0.0499999523162842 0.000979547388851643
0.100000023841858 0.00175867509096861
0.149999976158142 0.00222270772792399
0.200000047683716 0.00328481174074113
0.25 0.00408124923706055
0.299999952316284 0.00478076841682196
};
\addlegendentry{Dopri5}

==> figs/stiff_dynamics/compute_time_data.tex <==
\definecolor{color0}{rgb}{1,1,0}
\definecolor{color1}{rgb}{1,0,1}

\addplot [ultra thick, blue, mark=asterisk, mark size=2, mark options={solid}]
table {%
0.0010000467300415 0.149672269821167
0.0399999618530273 0.172874704003334
0.0800000429153442 0.162971243262291
0.120000004768372 0.154009819030762
0.159999966621399 0.168834462761879
0.200000047683716 0.161410093307495
0.299999952316284 0.159499391913414
};
\addlegendentry{TLN, with \(\midpoint_{\nnParamsMidpoint}\) (ours)}
\addplot [ultra thick, red, mark=*, mark size=2, mark options={solid}]
table {%
0.0010000467300415 0.0606999360024929
0.0399999618530273 0.042940616607666
0.0800000429153442 0.0390698872506618
0.120000004768372 0.0375058650970459
0.159999966621399 0.038672212511301
0.200000047683716 0.0419867001473904
0.299999952316284 0.0395693741738796
};
\addlegendentry{Fixed-Step RK4}
\addplot [ultra thick, green!50.1960784313725!black, mark=+, mark size=2, mark options={solid}]
table {%
0.0010000467300415 0.0772705003619194
0.0399999618530273 0.369270741939545
0.0800000429153442 0.57939213514328
0.120000004768372 0.775398671627045
0.159999966621399 1.00783371925354
0.200000047683716 1.20596468448639
0.299999952316284 1.85655772686005
};
\addlegendentry{Adaptive-Step RK4}
\addplot [ultra thick, cyan, mark=square, mark size=2, mark options={solid}]
table {%
0.0010000467300415 0.0498607195913792
0.0399999618530273 0.0567822530865669
0.0800000429153442 0.0505330599844456
0.120000004768372 0.0559322834014893
0.159999966621399 0.0483756102621555
0.200000047683716 0.0538115501403809
0.299999952316284 0.0522339344024658
};
\addlegendentry{TLN, no \(\midpoint_{\nnParamsMidpoint}\)}
\addplot [ultra thick, color1, mark=diamond, mark size=2, mark options={solid}]
table {%
0.0010000467300415 0.273075819015503
0.0399999618530273 0.295884847640991
0.0800000429153442 0.170989528298378
0.120000004768372 0.168870240449905
0.159999966621399 0.153860062360764
0.200000047683716 0.161334529519081
0.299999952316284 0.155106991529465
};
\addlegendentry{Hypersolver}

% \addplot [ultra thick, blue, mark=asterisk, mark size=2, mark options={solid}]
% table {%
% 0.0010000467300415 0.0010607244912535
% 0.0399999618530273 0.000973462883848697
% 0.0800000429153442 0.000989913707599044
% 0.120000004768372 0.00106740009505302
% 0.159999966621399 0.00106596946716309
% 0.200000047683716 0.00100064254365861
% 0.299999952316284 0.000990391010418534
% };
% \addlegendentry{Taylor-Lagrange Method (Ours)}
% \addplot [ultra thick, red, mark=*, mark size=2, mark options={solid}]
% table {%
% 0.0010000467300415 0.000273466081125662
% 0.0399999618530273 0.000261783658061177
% 0.0800000429153442 0.000256061495747417
% 0.120000004768372 0.000271320372121409
% 0.159999966621399 0.000274181336862966
% 0.200000047683716 0.000253439007792622
% 0.299999952316284 0.000257253646850586
% };
% \addlegendentry{Fixed Step RK4}
% \addplot [ultra thick, green!50.1960784313725!black, mark=+, mark size=2, mark options={solid}]
% table {%
% 0.0010000467300415 0.000785350683145225
% 0.0399999618530273 0.00225615524686873
% 0.0800000429153442 0.00397300766780972
% 0.120000004768372 0.0061814789660275
% 0.159999966621399 0.00745534943416715
% 0.200000047683716 0.00853395648300648
% 0.299999952316284 0.0129771251231432
% };
% \addlegendentry{Adaptive Step RK4}

==> figs/stiff_dynamics/errormean_data.tex <==
\definecolor{color0}{rgb}{1,1,0}
\definecolor{color1}{rgb}{1,0,1}

\path [draw=blue, fill=blue, opacity=0.35]
(axis cs:0.001,1.22432231607065e-05)
--(axis cs:0.001,7.0226525718298e-06)
--(axis cs:0.101,1.57913161348934e-05)
--(axis cs:0.201,1.92354575409531e-05)
--(axis cs:0.301,2.26721727960268e-05)
--(axis cs:0.401,2.61100725720084e-05)
--(axis cs:0.501,2.95577586774098e-05)
--(axis cs:0.601,3.30237601137563e-05)
--(axis cs:0.701,3.65164718199735e-05)
--(axis cs:0.801,4.00440981940018e-05)
--(axis cs:0.901,4.36146031258025e-05)
--(axis cs:1.001,4.72356678031217e-05)
--(axis cs:1.101,5.09146569179507e-05)
--(axis cs:1.201,5.46585935672979e-05)
--(axis cs:1.301,5.84741423971278e-05)
--(axis cs:1.401,6.23676004854888e-05)
--(axis cs:1.501,6.634489500766e-05)
--(axis cs:1.601,7.04115867021567e-05)
--(axis cs:1.701,7.45728780235537e-05)
--(axis cs:1.801,7.88336250379798e-05)
--(axis cs:1.901,8.31983519207051e-05)
--(axis cs:1.901,0.000157596788438418)
--(axis cs:1.901,0.000157596788438418)
--(axis cs:1.801,0.000153167335697786)
--(axis cs:1.701,0.000148843200539492)
--(axis cs:1.601,0.000144619927717731)
--(axis cs:1.501,0.000140492737528351)
--(axis cs:1.401,0.000136456512135098)
--(axis cs:1.301,0.000132505784648453)
--(axis cs:1.201,0.000128634731836257)
--(axis cs:1.101,0.000124837171478952)
--(axis cs:1.001,0.00012110656532286)
--(axis cs:0.901,0.000117436028555871)
--(axis cs:0.801,0.000113818346583337)
--(axis cs:0.701,0.00011024599960211)
--(axis cs:0.601,0.000106711195143202)
--(axis cs:0.501,0.000103205908311338)
--(axis cs:0.401,9.97219289777816e-05)
--(axis cs:0.301,9.62509147209766e-05)
--(axis cs:0.201,9.27844478620904e-05)
--(axis cs:0.101,8.93140946583607e-05)
--(axis cs:0.001,1.22432231607065e-05)
--cycle;

\path [draw=green!50.1960784313725!black, fill=green!50.1960784313725!black, opacity=0.35]
(axis cs:0.001,1.78254517155225e-08)
--(axis cs:0.001,1.02048062518124e-08)
--(axis cs:0.101,7.21230249529959e-07)
--(axis cs:0.201,1.52432634729895e-06)
--(axis cs:0.301,2.38686223890924e-06)
--(axis cs:0.401,3.31315980797638e-06)
--(axis cs:0.501,4.30784151600818e-06)
--(axis cs:0.601,5.37585100965673e-06)
--(axis cs:0.701,6.52247465201333e-06)
--(axis cs:0.801,7.75336475966375e-06)
--(axis cs:0.901,9.07456460856542e-06)
--(axis cs:1.001,1.04925351278503e-05)
--(axis cs:1.101,1.20141832070472e-05)
--(axis cs:1.201,1.36468921120239e-05)
--(axis cs:1.301,1.53985539586486e-05)
--(axis cs:1.401,1.72776046925548e-05)
--(axis cs:1.501,1.92930614508232e-05)
--(axis cs:1.601,2.14545626012113e-05)
--(axis cs:1.701,2.37724109571475e-05)
--(axis cs:1.801,2.62576198310577e-05)
--(axis cs:1.901,2.8921962839584e-05)
--(axis cs:1.901,0.0013758367999806)
--(axis cs:1.901,0.0013758367999806)
--(axis cs:1.801,0.00124899914588345)
--(axis cs:1.701,0.00113068928454167)
--(axis cs:1.601,0.00102034672035594)
--(axis cs:1.501,0.000917447155954296)
--(axis cs:1.401,0.000821500122460741)
--(axis cs:1.301,0.0007320467780878)
--(axis cs:1.201,0.000648657856731224)
--(axis cs:1.101,0.00057093175966268)
--(axis cs:1.001,0.000498492776866924)
--(axis cs:0.901,0.000430989426213599)
--(axis cs:0.801,0.00036809290386072)
--(axis cs:0.701,0.000309495636302639)
--(axis cs:0.601,0.000254909926851561)
--(axis cs:0.501,0.000204066690291127)
--(axis cs:0.401,0.00015671426831654)
--(axis cs:0.301,0.000112617322976165)
--(axis cs:0.201,7.15558016509271e-05)
--(axis cs:0.101,3.33239884908318e-05)
--(axis cs:0.001,1.78254517155225e-08)
--cycle;

\path [draw=red, fill=red, opacity=0.35]
(axis cs:0.001,0.00809140261179106)
--(axis cs:0.001,0.00465580662539734)
--(axis cs:0.101,0.0083004063811262)
--(axis cs:0.201,0.00830040638119938)
--(axis cs:0.301,0.00830040638129465)
--(axis cs:0.401,0.00830040638143935)
--(axis cs:0.501,0.00830040638163991)
--(axis cs:0.601,0.0083004063818777)
--(axis cs:0.701,0.00830040638216954)
--(axis cs:0.801,0.00830040638251061)
--(axis cs:0.901,0.00830040638286883)
--(axis cs:1.001,0.00830040638324899)
--(axis cs:1.101,0.00830040638366369)
--(axis cs:1.201,0.00830040638414179)
--(axis cs:1.301,0.00830040638466442)
--(axis cs:1.401,0.00830040638520852)
--(axis cs:1.501,0.00830040638577212)
--(axis cs:1.601,0.00830040638638766)
--(axis cs:1.701,0.0083004063870621)
--(axis cs:1.801,0.00830040638777051)
--(axis cs:1.901,0.00830040638847738)
--(axis cs:1.901,0.0578380604654673)
--(axis cs:1.901,0.0578380604654673)
--(axis cs:1.801,0.0578380604646888)
--(axis cs:1.701,0.0578380604639543)
--(axis cs:1.601,0.057838060463265)
--(axis cs:1.501,0.0578380604626203)
--(axis cs:1.401,0.0578380604620163)
--(axis cs:1.301,0.0578380604614546)
--(axis cs:1.201,0.0578380604609344)
--(axis cs:1.101,0.0578380604604532)
--(axis cs:1.001,0.0578380604600144)
--(axis cs:0.901,0.0578380604596175)
--(axis cs:0.801,0.0578380604592626)
--(axis cs:0.701,0.0578380604589516)
--(axis cs:0.601,0.0578380604586808)
--(axis cs:0.501,0.0578380604584513)
--(axis cs:0.401,0.0578380604582643)
--(axis cs:0.301,0.0578380604581133)
--(axis cs:0.201,0.0578380604580009)
--(axis cs:0.101,0.0578380604579231)
--(axis cs:0.001,0.00809140261179106)
--cycle;

\path [draw=color0, fill=cyan, opacity=0.35]
(axis cs:0.001,0.132494172682365)
--(axis cs:0.001,0.0823046266827903)
--(axis cs:0.101,0.191462927704687)
--(axis cs:0.201,0.191464191151929)
--(axis cs:0.301,0.191466288557732)
--(axis cs:0.401,0.191469219922107)
--(axis cs:0.501,0.191472985245045)
--(axis cs:0.601,0.191477584526581)
--(axis cs:0.701,0.19148301776671)
--(axis cs:0.801,0.191489284965421)
--(axis cs:0.901,0.19149638612272)
--(axis cs:1.001,0.191504321238606)
--(axis cs:1.101,0.191513090313058)
--(axis cs:1.201,0.191522693346096)
--(axis cs:1.301,0.191533130337721)
--(axis cs:1.401,0.191544401287933)
--(axis cs:1.501,0.191556506196718)
--(axis cs:1.601,0.191569445064074)
--(axis cs:1.701,0.191583217890045)
--(axis cs:1.801,0.191597824674582)
--(axis cs:1.901,0.191613265417724)
--(axis cs:1.901,1.24796823431708)
--(axis cs:1.901,1.24796823431708)
--(axis cs:1.801,1.24795279357381)
--(axis cs:1.701,1.24793818678912)
--(axis cs:1.601,1.24792441396302)
--(axis cs:1.501,1.2479114750955)
--(axis cs:1.401,1.24789937018655)
--(axis cs:1.301,1.24788809923619)
--(axis cs:1.201,1.24787766224441)
--(axis cs:1.101,1.24786805921121)
--(axis cs:1.001,1.2478592901366)
--(axis cs:0.901,1.24785135502056)
--(axis cs:0.801,1.24784425386311)
--(axis cs:0.701,1.24783798666425)
--(axis cs:0.601,1.24783255342397)
--(axis cs:0.501,1.24782795414227)
--(axis cs:0.401,1.24782418881917)
--(axis cs:0.301,1.24782125745466)
--(axis cs:0.201,1.24781916004873)
--(axis cs:0.101,1.24781789660138)
--(axis cs:0.001,0.132494172682365)
--cycle;

\path [draw=color1, fill=color1, opacity=0.35]
(axis cs:0.001,0.00044395971224918)
--(axis cs:0.001,0.000202376699349458)
--(axis cs:0.101,0.00174089326885774)
--(axis cs:0.201,0.00601500417312637)
--(axis cs:0.301,0.0142474846960112)
--(axis cs:0.401,0.0240981615730067)
--(axis cs:0.501,0.037105388740629)
--(axis cs:0.601,0.0536268571817205)
--(axis cs:0.701,0.0740427762088891)
--(axis cs:0.801,0.0987655842398214)
--(axis cs:0.901,0.128244733395499)
--(axis cs:1.001,0.162971711002568)
--(axis cs:1.101,0.203485374900346)
--(axis cs:1.201,0.250377674893471)
--(axis cs:1.301,0.304299831765615)
--(axis cs:1.401,0.365969046377169)
--(axis cs:1.501,0.436175813920025)
--(axis cs:1.601,0.515791922146263)
--(axis cs:1.701,0.605779217200358)
--(axis cs:1.801,0.707199226504289)
--(axis cs:1.901,0.821223734944082)
--(axis cs:1.901,39.4665351082174)
--(axis cs:1.901,39.4665351082174)
--(axis cs:1.801,33.0608396728298)
--(axis cs:1.701,27.6534112308936)
--(axis cs:1.601,23.0644868527758)
--(axis cs:1.501,19.1565938203508)
--(axis cs:1.401,15.822211342056)
--(axis cs:1.301,12.9756288492796)
--(axis cs:1.201,10.5474088584803)
--(axis cs:1.101,8.48051618434833)
--(axis cs:1.001,6.72754509797702)
--(axis cs:0.901,5.24868944261963)
--(axis cs:0.801,4.01022759180381)
--(axis cs:0.701,2.98337180777668)
--(axis cs:0.601,2.14338039822873)
--(axis cs:0.501,1.46886246871943)
--(axis cs:0.401,0.941225478992996)
--(axis cs:0.301,0.544228578907788)
--(axis cs:0.201,0.263609646840376)
--(axis cs:0.101,0.0867370654555806)
--(axis cs:0.001,0.00044395971224918)
--cycle;

\addplot [ultra thick, blue]
table {%
0.0010000467300415 9.63294132816372e-06
0.10099995136261 4.57040368928574e-05
0.200999975204468 4.91526479891036e-05
0.300999999046326 5.25936666235793e-05
0.401000022888184 5.60356711503118e-05
0.500999927520752 5.94873417867348e-05
0.601000070571899 6.29570131422952e-05
0.700999975204468 6.64532126393169e-05
0.800999999046326 6.99840093147941e-05
0.901000022888184 7.35574649297632e-05
1.00100004673004 7.71812337916344e-05
1.10099995136261 8.08626064099371e-05
1.20099997520447 8.46087714307941e-05
1.30099999904633 8.84261826286092e-05
1.40100002288818 9.2321315605659e-05
1.50100004673004 9.63000202318653e-05
1.60099995136261 0.000100367942650337
1.70099997520447 0.000104530205135234
1.80099999904633 0.000108791777165607
1.90100002288818 0.000113157046143897
};
% \addlegendentry{TayLa}
\addplot [ultra thick, green!50.1960784313725!black]
table {%
0.0010000467300415 1.40151223959606e-08
0.10099995136261 6.77506614010781e-06
0.200999975204468 1.44774066939135e-05
0.300999999046326 2.27498439926421e-05
0.401000022888184 3.16337864205707e-05
0.500999927520752 4.11735927627888e-05
0.601000070571899 5.14166677021421e-05
0.700999975204468 6.24137101112865e-05
0.800999999046326 7.42189586162567e-05
0.901000022888184 8.68903443915769e-05
1.00100004673004 0.000100489844044205
1.10099995136261 0.000115083734272048
1.20099997520447 0.000130742686451413
1.30099999904633 0.000147542596096173
1.40100002288818 0.000165564211783931
1.50100004673004 0.000184894059202634
1.60099995136261 0.000205624717636965
1.70099997520447 0.000227854659897275
1.80099999904633 0.000251689896686003
1.90100002288818 0.000277243147138506
};
% \addlegendentry{ODEInt}
\addplot [ultra thick, red]
table {%
0.0010000467300415 0.00637360569089651
0.10099995136261 0.0284512173384428
0.200999975204468 0.0284512173384428
0.300999999046326 0.0284512173384428
0.401000022888184 0.0284512173384428
0.500999927520752 0.0284512173384428
0.601000070571899 0.0284512173384428
0.700999975204468 0.0284512173384428
0.800999999046326 0.0284512173384428
0.901000022888184 0.0284512173384428
1.00100004673004 0.0284512173384428
1.10099995136261 0.0284512173384428
1.20099997520447 0.0284512173384428
1.30099999904633 0.0284512173384428
1.40100002288818 0.0284512173384428
1.50100004673004 0.0284512173384428
1.60099995136261 0.0284512173384428
1.70099997520447 0.0284512173384428
1.80099999904633 0.0284512173384428
1.90100002288818 0.0284512173384428
};
% \addlegendentry{RK4}
\addplot [semithick, cyan]
table {%
0.0010000467300415 0.107399389147758
0.10099995136261 0.635387599468231
0.200999975204468 0.635388791561127
0.300999999046326 0.635390877723694
0.401000022888184 0.635393857955933
0.500999927520752 0.635397493839264
0.601000070571899 0.635402202606201
0.700999975204468 0.635407626628876
0.800999999046326 0.635413885116577
0.901000022888184 0.635420858860016
1.00100004673004 0.635428905487061
1.10099995136261 0.635437607765198
1.20099997520447 0.635447382926941
1.30099999904633 0.635457694530487
1.40100002288818 0.635469019412994
1.50100004673004 0.635481059551239
1.60099995136261 0.63549417257309
1.70099997520447 0.635507762432098
1.80099999904633 0.635522425174713
1.90100002288818 0.635537922382355
};
% \addlegendentry{Taylor}
\addplot [ultra thick, color1]
table {%
0.0010000467300415 0.000323168293107301
0.10099995136261 0.0178503561764956
0.200999975204468 0.0525726787745953
0.300999999046326 0.107933595776558
0.401000022888184 0.186255887150764
0.500999927520752 0.29012256860733
0.601000070571899 0.422425657510757
0.700999975204468 0.586414992809296
0.800999999046326 0.785754382610321
0.901000022888184 1.02458918094635
1.00100004673004 1.30762755870819
1.10099995136261 1.64024186134338
1.20099997520447 2.02859473228455
1.30099999904633 2.47980356216431
1.40100002288818 3.00214982032776
1.50100004673004 3.60536408424377
1.60099995136261 4.30100727081299
1.70099997520447 5.10302066802979
1.80099999904633 6.02849721908569
1.90100002288818 7.09886455535889
};
% \addlegendentry{HyperEuler}

==> figs/stiff_dynamics/geommean_data.tex <==
\definecolor{color0}{rgb}{1,1,0}
\definecolor{color1}{rgb}{1,0,1}

\path [draw=blue, fill=blue, opacity=0.35]
(axis cs:0.001,8.33947368368458e-05)
--(axis cs:0.001,1.24749984623545e-05)
--(axis cs:0.04,0.000148284192171244)
--(axis cs:0.08,0.00121863789056725)
--(axis cs:0.12,0.00431843944312736)
--(axis cs:0.16,0.0106152578689839)
--(axis cs:0.2,0.0214027422780434)
--(axis cs:0.3,0.0782023744040138)
--(axis cs:0.3,0.0854298889921838)
--(axis cs:0.3,0.0854298889921838)
--(axis cs:0.2,0.0222224912552081)
--(axis cs:0.16,0.0114059295059533)
--(axis cs:0.12,0.00561428830732961)
--(axis cs:0.08,0.00126036626556441)
--(axis cs:0.04,0.000205437202844882)
--(axis cs:0.001,8.33947368368458e-05)
--cycle;

\path [draw=green!50.1960784313725!black, fill=green!50.1960784313725!black, opacity=0.35]
(axis cs:0.001,6.00415255218138e-07)
--(axis cs:0.001,3.37411873006559e-08)
--(axis cs:0.04,2.64744128551148e-07)
--(axis cs:0.08,3.14177771787722e-07)
--(axis cs:0.12,2.04274855720507e-07)
--(axis cs:0.16,2.13507623333703e-07)
--(axis cs:0.2,2.53912487477593e-07)
--(axis cs:0.3,4.23077427236018e-07)
--(axis cs:0.3,2.0140964786787e-05)
--(axis cs:0.3,2.0140964786787e-05)
--(axis cs:0.2,1.20876853764626e-05)
--(axis cs:0.16,1.01641531897253e-05)
--(axis cs:0.12,9.7246113264763e-06)
--(axis cs:0.08,1.49566507101769e-05)
--(axis cs:0.04,1.26033308289206e-05)
--(axis cs:0.001,6.00415255218138e-07)
--cycle;

\path [draw=red, fill=red, opacity=0.35]
(axis cs:0.001,0.055895304165353)
--(axis cs:0.001,0.00825412966993772)
--(axis cs:0.04,6.99999287874047)
--(axis cs:0.08,6.99999959245489)
--(axis cs:0.12,6.99999992390559)
--(axis cs:0.16,6.99999997705648)
--(axis cs:0.2,6.99999999101535)
--(axis cs:0.3,6.99999999840472)
--(axis cs:0.3,6.99999999955855)
--(axis cs:0.3,6.99999999955855)
--(axis cs:0.2,6.99999999751374)
--(axis cs:0.16,6.99999999365099)
--(axis cs:0.12,6.9999999789429)
--(axis cs:0.08,6.99999988722274)
--(axis cs:0.04,6.99999802937384)
--(axis cs:0.001,0.055895304165353)
--cycle;

\path [draw=cyan, fill=cyan, opacity=0.35]
(axis cs:0.001,1.11863569133114)
--(axis cs:0.001,0.187915215004402)
--(axis cs:0.04,6.99909392193158)
--(axis cs:0.08,6.99978784249982)
--(axis cs:0.12,6.99991016492254)
--(axis cs:0.16,6.99995165252201)
--(axis cs:0.2,6.99997034552299)
--(axis cs:0.3,6.99998811429554)
--(axis cs:0.3,6.99999671092728)
--(axis cs:0.3,6.99999671092728)
--(axis cs:0.2,6.99999179378199)
--(axis cs:0.16,6.99998662077201)
--(axis cs:0.12,6.9999751393175)
--(axis cs:0.08,6.99994128425491)
--(axis cs:0.04,6.99974914285832)
--(axis cs:0.001,1.11863569133114)
--cycle;

\path [draw=color1, fill=color1, opacity=0.35]
(axis cs:0.001,0.00482898743131399)
--(axis cs:0.001,0.000550920778393633)
--(axis cs:0.04,4.2125657031136)
--(axis cs:0.08,6.33167146140867)
--(axis cs:0.12,6.85350710694458)
--(axis cs:0.16,6.91675245428209)
--(axis cs:0.2,6.93992851966144)
--(axis cs:0.3,6.96948001831172)
--(axis cs:0.3,6.99256890993118)
--(axis cs:0.3,6.99256890993118)
--(axis cs:0.2,6.9846105822864)
--(axis cs:0.16,6.97760944349158)
--(axis cs:0.12,6.96014117465528)
--(axis cs:0.08,6.99880329390625)
--(axis cs:0.04,5.97781506101105)
--(axis cs:0.001,0.00482898743131399)
--cycle;

\addplot [ultra thick, blue, mark=asterisk, mark size=2, mark options={solid}]
table {%
0.0010000467300415 4.18408635596279e-05
0.0399999618530273 0.000156951253302395
0.0800000429153442 0.00122368626762182
0.120000004768372 0.00451629003509879
0.159999966621399 0.0107208294793963
0.200000047683716 0.0215205121785402
0.299999952316284 0.0791841298341751
};
% \addlegendentry{TayLa}
\addplot [ultra thick, green!50.1960784313725!black, mark=+, mark size=2, mark options={solid}]
table {%
0.0010000467300415 1.81246761599141e-07
0.0399999618530273 2.53911366598913e-06
0.0800000429153442 3.01322506857105e-06
0.120000004768372 1.95916209122515e-06
0.159999966621399 2.04771163225814e-06
0.200000047683716 2.43522981691058e-06
0.299999952316284 4.05766650146688e-06
};
% \addlegendentry{ODEInt}
\addplot [ultra thick, red, mark=*, mark size=2, mark options={solid}]
table {%
0.0010000467300415 0.0280063692480326
0.0399999618530273 6.99999570846558
0.0800000429153442 6.99999952316284
0.120000004768372 6.99999952316284
0.159999966621399 6.99999952316284
0.200000047683716 6.99999952316284
0.299999952316284 6.99999952316284
};
% \addlegendentry{RK4}
\addplot [ultra thick, cyan, mark=square, mark size=2, mark options={solid}]
table {%
0.0010000467300415 0.603210389614105
0.0399999618530273 6.99942111968994
0.0800000429153442 6.99986505508423
0.120000004768372 6.9999418258667
0.159999966621399 6.99996900558472
0.200000047683716 6.99998044967651
0.299999952316284 6.99999189376831
};
% \addlegendentry{Taylor}
\addplot [ultra thick, color1, mark=diamond, mark size=2, mark options={solid}]
table {%
0.0010000467300415 0.00206716358661652
0.0399999618530273 5.09519100189209
0.0800000429153442 6.70267534255981
0.120000004768372 6.90682506561279
0.159999966621399 6.94718027114868
0.200000047683716 6.9622688293457
0.299999952316284 6.98102426528931
};
% \addlegendentry{HyperEuler}


==> figs/stiff_dynamics/trajxy_data.tex <==
\definecolor{color0}{rgb}{1,1,0}
\definecolor{color1}{rgb}{1,0,1}

\addplot [ultra thick, color1, mark=diamond, mark size=4, mark options={solid}]
table {%
0.159471392631531 0.292764902114868
0.0203226804733276 0.222977876663208
-0.0308550596237183 0.197178840637207
-0.0496714115142822 0.187559366226196
-0.0565663576126099 0.183900117874146
-0.0590687990188599 0.182437062263489
-0.0599527359008789 0.181783437728882
-0.0602402687072754 0.181428074836731
-0.0603080987930298 0.181182861328125
-0.0602520704269409 0.18078875541687
-0.0598421096801758 0.179523110389709
-0.0597225427627563 0.17916464805603
};
% \addlegendentry{HyperEuler}
\addplot [ultra thick, cyan, , mark=square, mark size=2, mark options={solid}]
table {%
0.159471392631531 0.292764902114868
0.0493637323379517 0.237498164176941
-0.00565969944000244 0.209773778915405
-0.033141016960144 0.195820569992065
-0.0468515157699585 0.188753128051758
-0.0536763668060303 0.185128569602966
-0.057058572769165 0.183225512504578
-0.0587195158004761 0.182183504104614
-0.0595197677612305 0.181571841239929
-0.0598897933959961 0.181175708770752
-0.0600446462631226 0.180887222290039
-0.0600920915603638 0.180652737617493
-0.0600525140762329 0.180251598358154
-0.059837818145752 0.179519414901733
-0.0597195625305176 0.179160118103027
};
% \addlegendentry{Taylor}
\addplot [ultra thick, green!50.1960784313725!black, mark=+, mark size=4, mark options={solid}]
table {%
0.159471392631531 0.292764902114868
0.0202527046203613 0.222942709922791
-0.0309245586395264 0.197141289710999
-0.0497132539749146 0.18753445148468
-0.0565868616104126 0.183885335922241
-0.059077262878418 0.182428121566772
-0.0599552392959595 0.181777238845825
-0.0602400302886963 0.181423187255859
-0.0603065490722656 0.181178450584412
-0.060249924659729 0.180784583091736
-0.0598394870758057 0.179518580436707
-0.0597199201583862 0.179159879684448
};
% \addlegendentry{ODEint}
\addplot [ultra thick, red, mark=*, mark size=2, mark options={solid}]
table {%
0.159471392631531 0.292764902114868
0.0218216180801392 0.223727107048035
-0.0297590494155884 0.197724103927612
-0.0490638017654419 0.187859177589417
-0.0562652349472046 0.184046149253845
-0.0589280128479004 0.182502746582031
-0.0598886013031006 0.18181049823761
-0.060211181640625 0.181437611579895
-0.0602943897247314 0.181184649467468
-0.0602477788925171 0.180785655975342
-0.0598993301391602 0.17969822883606
-0.0597199201583862 0.179159879684448
};
% \addlegendentry{RK4}
\addplot [ultra thick, blue, mark=asterisk, mark size=2, mark options={solid}]
table {%
0.159471392631531 0.292764902114868
0.0202503204345703 0.222941517829895
-0.0309262275695801 0.197140455245972
-0.049714207649231 0.187533974647522
-0.0565873384475708 0.183885097503662
-0.0590775012969971 0.182428002357483
-0.059955358505249 0.181777238845825
-0.0602400302886963 0.181423187255859
-0.0603066682815552 0.181178450584412
-0.060249924659729 0.180784583091736
-0.0598394870758057 0.179518580436707
-0.0597199201583862 0.179159879684448
};
% \addlegendentry{Tayla}

==> tex/00_abstract_v1.tex <==
\begin{abstract}
    Neural ordinary differential equations (neural ODEs) -- parametrizations of differential equations using neural networks -- have shown tremendous promise in learning models of unknown continuous-time dynamical systems from data.
    However, each training step of a NODE requires numerical integration of the underlying neural network, making training prohibitively expensive in practice.
    Indeed, existing methods for training neural ODEs rely on off-the-shelf adaptive step-size numerical integration schemes, which often require an excessive number of neural network evaluations to obtain sufficient accuracy.
    By contrast, we accelerate the training of neural ODEs by proposing a data-driven approach to numerical integration which requires only a fixed number of neural network evaluations while ensuring little-to-no loss in the integrator's accuracy.
    The proposed approach uses a fixed-order Taylor-Lagrange expansion to integrate the neural ODE, while also estimating the expansion's approximation error.
    We provide an efficient method to estimate this approximation error, by learning the so-called midpoint value of the expansion.
    As a result, the proposed approach achieves the same accuracy as adaptive step-size schemes while employing only low-order Taylor-Lagrange expansions, thus greatly reducing the computational cost of integration.
    We provide a theoretical upper bound on the error of the proposed Taylor-Lagrange expansion, in terms of the approximation error of the midpoint.
    Through a series of experiments, including supervised classification, learning generative models, and learning robotic system dynamics, the proposed approach trains neural ODEs ten times faster than state-of-the-art approaches, while being marginally less accurate.
    \color{red}
    Fix the empirical results numbers.
    \color{black}
\end{abstract}

==> tex/00_abstract_v2.tex <==
\begin{abstract}
    Neural ordinary differential equations (NODEs) -- parametrizations of differential equations using neural networks -- have shown tremendous promise in learning models of unknown continuous-time dynamical systems from data.
    However, every forward evaluation of a NODE requires numerical integration of the neural network used to capture the system dynamics, making their training prohibitively expensive.
    % used to parametrize the ODE.
    % This requirement makes the repeated evaluation, and resultingly the training, of NODEs prohibitively expensive.
    % and the repeated evaluation of NODEs prohibitively expensive.
    % However, each training step of a NODE requires numerical integration of the underlying neural network, making training prohibitively expensive in practice.
    Existing works rely on off-the-shelf adaptive step-size numerical integration schemes, which often require an excessive number of evaluations of the underlying dynamics network to obtain sufficient accuracy for training.
    % Existing methods for the evaluation of NODEs rely on off-the-shelf adaptive step-size numerical integration schemes, which often require an excessive number of neural network evaluations to obtain sufficient accuracy.
    % Indeed, existing methods for training NODEs rely on off-the-shelf adaptive step-size numerical integration schemes, which often require an excessive number of neural network evaluations to obtain sufficient accuracy.
    By contrast, we accelerate the evaluation and the training of NODEs by proposing a data-driven approach to their numerical integration.
    % which requires only a fixed number of evaluations of the dynamics network while enjoying little-to-no loss in the integrator's accuracy.
    % We accordingly present both a methodology and practical training algorithms to use fixed-order Taylor expansions to evaluate the NODE, while also estimating the expansion's approximation error.
    The proposed Taylor-Lagrange NODEs (TL-NODEs) use a fixed-order Taylor expansion for numerical integration, while also learning to estimate the expansion's approximation error.
    % We provide an efficient method to estimate this approximation error by learning the so-called midpoint value of the expansion, as well as a theoretical upper bound on the error of the Taylor expansion, in terms of the approximation error of the midpoint.
    % We provide an efficient method to estimate this approximation error by learning the so-called midpoint value of the expansion.
    As a result, the proposed approach achieves the same accuracy as adaptive step-size schemes while employing only low-order Taylor expansions, thus greatly reducing the computational cost necessary to integrate the NODE.
    A suite of numerical experiments, including modeling dynamical systems, image classification, and density estimation, demonstrate that TL-NODEs can be trained more than an order of magnitude faster than state-of-the-art approaches, without any loss in performance.
    % proposed TL-NODEs trains neural ODEs ten times faster than state-of-the-art approaches, while being marginally less accurate.
    % % We provide a theoretical upper bound on the error of the proposed Taylor expansion, in terms of the approximation error of the midpoint.
    % \color{red}
    % A suite of numerical experiments, including modeling dynamical systems, image classification, and density estimation, demonstrate that the proposed approach trains neural ODEs ten times faster than state-of-the-art approaches, while being marginally less accurate.
    % \color{black}
    
\end{abstract}

==> tex/01_intro_v1.tex <==
\section{Introduction}

Neural ordinary differential equations (neural ODEs) have recently shown tremendous promise as a means to learn unknown continuous-time dynamical systems from trajectory data \cite{chen2018neural}.
By parametrizing differential equations as neural networks, as opposed to directly fitting the available trajectory data, neural ODEs provide compact representations of continuous-time systems that are memory-efficient and that are well understood; they allow the user to harness an existing wealth of knowledge from applied mathematics, physics, and engineering.
For example, a number of recent works have used neural ODEs as a means to incorporate physics-based knowledge into the learning of dynamical systems models~\cite{djeumou2021neural,menda2019structured,gupta2020structured,duong2021hamiltonian,cranmer2020lagrangian,greydanus2019hamiltonian,finzi2020simplifying,zhong2020dissipative,roehrl2020modeling,zhong2021benchmarking}.
Furthermore, neural ODEs have been used to define continuous normalizing flows -- a class of invertible density models -- for the learning of complex probability distributions over data \cite{chen2018neural,grathwohl2018ffjord,mathieu2020riemannian,salman2018deep}.

However, the training of neural ODEs can become prohibitively expensive \cite{grathwohl2018ffjord,kelly2020learning,Finlay2020HowTT}.
In particular, every iteration of the training procedure requires the numerical integration of the neural network parameterizing the dynamics.
Existing methods for the training of neural ODEs use off-the-shelf adaptive step-size numerical integration schemes for this purpose.
However, such integration schemes have been shown in practice to require an excessive number of neural network evaluations to obtain sufficient accuracy.
% In particular, each training step of a neural ODE requires the numerical integration of the underlying neural network.
% Existing neural ODE training methods use off-the-shelf adaptive step-size numerical integration schemes, which have been shown in practice to require an excessive number of neural network evaluations in order to obtain sufficient accuracy.
Furthermore, the severity of this problem has been shown to grow as the training of the neural ODE progresses; while the neural ODE learns to fit the available data, it does not learn a representation of the dynamics that is easy to integrate \cite{Finlay2020HowTT}.
These computational issues render the training of neural ODEs on large datasets intractable, and they also prevent neural ODEs from being deployed in applications requiring fast online predictions; such as for model-predictive control of robotic systems.
% These computational issues make it intractable to train neural ODEs on large datasets, and prevent neural ODEs from being deployed on systems that require fast online predictions; such as model-predictive control of robotic systems.

In this work, we address the above issues by proposing a method to accelerate the training of neural ODEs.
More specifically, we propose a data-driven approach to numerical integration.
This approach requires only a fixed number of neural network evaluations, while ensuring little-to-no-loss in the integrator's accuracy.
% we accelerate the training of neural ODEs by proposing a data-driven approach to numerical integration which requires only a fixed number of neural network evaluations, while ensuring little-to-no loss in the integrator's accuracy.
% In particular, we propose the following three-step approach for the training of neural ODEs.
We detail the three major components of the proposed approach below.

% \begin{enumerate}
%     \item 
    \textbf{(1) Taylor-Lagrange method for the numerical integration of the neural ODE.}
    In order to integrate the neural ODE, we use a fixed-order Taylor-Lagrange expansion of the dynamical system in time.
    We take advantage of Taylor-mode automatic differentiation to efficiently compute the higher-order terms of the expansion on a GPU \cite{Bettencourt2019TaylorModeAD}.
    By specifying the number of terms to include in the expansion, we ensure that only a fixed number of evaluations of the neural network are required per training step, 
    % which greatly reduces the computation time for numerical integration.
    while also providing an expression for the approximation error of the numerical integration.
    
    % \item 
    \textbf{(2) Learning to predict the approximation error of the Taylor-Lagrange expansion.}
    In order to obtain more accurate numerical integration results than would typically be possible with a given expansion order, we estimate the expansion's approximation error as a function of the system's state and the size of the expansion time step.
    % We additionally learn to predict the approximation error of the truncated expansion, as a function of the system's state and the size of the expansion time step.
    To estimate this approximation error efficiently, we propose a method that learns to predict the so-called midpoint value -- a point near the center of the expansion at which the approximation error can be evaluated exactly.
    % While learning this midpoint value may be a complex task in general, we use explicit formulas for the midpoint in order to 
    % While learning this midpoint value may, in general, be as complex as learning the neural ODE itself, the proposed approach takes advantage of explicit formulas for the midpoint in order to re-use the information stored in the most current version of the neural ODE.
    While learning this midpoint value may, in general, be as complex as learning the neural ODE itself,
    we derive explicit formulas for the midpoint using assumptions on the regularity of the dynamics thus requiring only one unknown term in this expression to be learned.
    % the proposed approach takes advantage of explicit formulas for the midpoint which we derive using assumptions on the regularity of the dynamics.
    
    % Enforcing feasible approximation errors in the Taylor-Lagrange expansion.
    % \item 
    \textbf{(3) Regularizing the learned Taylor-Lagrange approximation error.}
    During the training of the neural ODE, we include two additional terms in the loss function beyond the prediction loss on trajectory data.
    Firstly, we penalize infeasible midpoint values; the midpoint value must lie between the center point and the prediction point of the expansion.
    Secondly, we use the magnitude of the predicted approximation error as a regularization term while training the neural ODE.
    This regularization term ensures that the predicted approximation error values are low, preventing the model from using this additional term to overfit the training data.
    % During the neural ODE's training, we propose additional terms in the loss function that penalize impossible midpoint values, and that regularize the loss using the magnitude of the predicted approximation error.
    % While training the neural ODE, we propose to add the magnitude of the approximation error as a regularization term in the loss function.
    
% \end{enumerate}

By using only fixed-order Taylor-Lagrange expansions to numerically integrate the ODE, the proposed approach requires only fixed numbers of evaluations of the underlying neural network, thus greatly reducing the computational cost of integration.
Meanwhile, by learning to predict the midpoint value of the expansion, the proposed approach achieves the same accuracy as adaptive step-size integration schemes.
% the proposed approach to numerical integration achieves the same accuracy as adaptive step-size integration schemes.
% Meanwhile, the proposed approach to numerical integration achieves the same accuracy as adaptive step-size integration schemes.
% the proposed approach requires only fixed numbers of evaluations of the underlying neural network, thus greatly reducing the computational cost of integration. 
We provide upper bounds on the error of the proposed Taylor-Lagrange expansion, in terms of the error in the predicted midpoint value and the order of the expansion.

% A suite of numerical experiments demonstrate the effectiveness of the proposed approach in accelerating the training of neural ODEs, without sacrificing the accuracy of the learned models.

We demonstrate the effectiveness of the proposed approach through several numerical experiments.
% for the integration of known stiff dynamics, as well as for density estimation tasks.
To demonstrate the benefits of estimating the expansion's approximation error, we use the proposed approach to integrate a known system with stiff dynamics.
For a fixed integration time step, the proposed Taylor-Lagrange integration scheme performs more accurately than Runge-Kutta methods, even when tested on points outside of the dataset used to train the approximation error predictor.
Through benchmark classification and density estimation tasks, we demonstrate that the proposed approach trains neural ODEs ten times faster than state-of-the-art approaches, while learning models that enjoy identical performance.
Across all of the experiments we observe that neural ODEs trained using the proposed Taylor-Lagrange numerical integrator require substantially fewer neural network evaluations than neural ODEs that were trained off-the-shelf adaptive step-size methods.
\color{red}
Add empirical results numbers to this paragraph.
\color{black}

% By applying the proposed data-driven numerical integration scheme to known systems with stiff dynamics, we observe the benefits provided by the proposed learning of the expansion's approximation error.
% In particular, for a fixed integration time step, the proposed Taylor-Lagrange integration scheme performs more accurately than Runge-Kutta methods, even when tested on points outside of the dataset used to train the approximation error estimator.
% training dataset.

% Through benchmark density estimation tasks, we demonstrate that the proposed approach trains neural ODEs ten times faster than state-of-the approaches, while the learned models enjoy identical performance.
% Finally, in all experiments we observe that neural ODEs trained using the proposed Taylor-Lagrange numerical integrator require substantially fewer neural network evaluations than neural ODEs that were trained off-the-shelf adaptive step-size methods.
% In other words, training the neural ODE using Taylor-series-based numerical integration and with the proposed error-related penalty terms results in a model that is easy to numerically integrate.

% When integrating known dynamics, we observe the gain in prediction accuracy of the proposed approach for learning to predict the expansion's approximation error; 
% integration of known stiff dynamics as well as density estimation tasks.



% \color{red}
% Remaining points to highlight through talking about numerical experiments.
% \begin{itemize}
%     \item The learning of the approximation error works. This was demonstrated using known dynamics.
%     \item We learn neural ODEs that are easier to solve while being just as accurate as other methods.
%     \item We learn neural ODEs much faster than other methods, while being just as (if not more) accurate.
%     \item We show results on complex robotics systems, demonstrating that we can be fast enough for online applications that were previously out of reach.
% \end{itemize}
% \color{black}

% \begin{itemize}
    % \item Neural ODEs are great.
    % \begin{itemize}
    %     \item Neural ordinary differential equations (neural ODEs) have shown tremendous promise in learning models of unknown continuous-time dynamical systems from data.
    %     These models, originally proposed by \citet{chen2018neural}, use neural networks to parametrize differential equations which are trained using 
    %     By parametrizing the differential equations that govern the system dynamics using neural networks, neural ODEs have demonstrated 
    %     Neural ODEs have been demonstrated to ...
    %     \item Neural ODE [Chen et al] has shown great promises in their ability to model unknown differential equations from trajectory data. For example, they enable to model unknown dynamical systems with prior physics knowledge \cite{djeumou2021neural} , learn dynamics of irregular time series, mean field games, \textcolor{blue}{continuous normalizing flow based generative models}, and more.
    % \end{itemize}
    
    % \item However, the training of neural ODEs is expensive.
    % \begin{itemize}
    %     \item However, the training of neural ODEs is often expensive.
    %     In particular, each training step of a neural ODE requires the numerical integration of differential equations represented by the underlying neural network.
    %     Existing approaches 
    %     \item \textcolor{red}{In particular, high–potential application domains for Neural ODEs such as control and prediction often deal with tight requirements on inference speed and computation e.g robotics (Hester, 2013) that are not currently within reach. For example, a generic state–of–the–art convolutional Neural ODE takes at least an order of magnitude2 longer to infer the label of a single MNIST image. This inefficiency results in inference passes far too slow for real–time applications.}
    %     \item Yet, some hurdles still remain [cite something]. In particular, although neural ODEs are memory efficient, they can take a prohibitively long time to train, which is arguably one of the main stumbling blocks towards their widespread adoption [Finlay et al]. 
    %     \item Specifically, training neural ODEs on large datasets has not been tractable due to the necessity of allowing the adaptive numerical ODE solver to refine (mainly due to learning complex ode) its step size to very small values [Finlay et al]. Thus, the adaptive solver requires an insane amount of time due to more and more functions evaluations, so more evaluations of a moderate-size neural network, in order to solve and terminate the training.
    % \end{itemize}
    
    % \item In this work, we solve this problem by proposing a data-driven approach to numerical integration which requires only a fixed number of neural network evaluations while ensuring little to no loss in the integrator's accuracy.
    % In particular, we propose a method for training neural ODEs that comprises the following distinct components.
    % \begin{enumerate}
    %     \item Taylor-Lagrange expansion to predict future states of the dynamical system.
    %     \begin{itemize}
    %         \item Such methods are used to quickly compute reach-sets in the safe control domain.
    %     \end{itemize}
    %     \item Estimating the approximation error by learning the midpoint value.
    %     \begin{itemize}
    %         \item Theoretically, even though such midpoint can be as complex as the vector field itself making it as hard to learn as the differential equations, we provide a theoretically-justified closed-form expression for the midpoint that reused the current estimate of the differential equation in order to simply its learning.
    %         \item Briefly talk about regularizing the midpoint value.
    %     \end{itemize}
    % \end{enumerate}
    
    % \item By learning the midpoint, we are able to achieve the same accuracy as adaptive step-size scemes while employing only low-order Taylor-Lagrange expansions, thus greatly reducing the computational cost of integration.
    % We provide upper bounds on the error of the proposed Taylor-Lagrange expansion, in terms of the approximation error of the midpoint.
    
    % \item Futhermore, ..., Paragraph outlining the problem of the increasing difficulty of solving neural ODEs as training increases when using adaptive solvers.
    % We solve this problem by regularizing the approximation error term, which is similar to regularizing the higher-order terms in the expansion, thus making the learned dynamics easier to solve.
    % \item Talk about the numerical results that show that the models we learn require less time steps than other approaches when using adaptive step-size solvers.
    
    % \item To demonstrate the effectiveness of the proposed learning of the midpoint value, we examine the ability of the proposed approach to learn estimations of the approximation error when the exact system dynamics are given.
    
    % \item We additionally use a suite of generative modeling benchmarks to exemplify the accelerated training of the proposed approach, while maintaining highly accurate predictions.
    
    % \item Finally, we show that the proposed approach could be used in high-dimensional robotics/airplane systems.
    % \begin{itemize}
    %     \item Bring this point back to the earlier motivation that we mentioned about needing fast learning and evaluation in order to do online control of cyberphysical systems.
    % \end{itemize}
    
% \end{itemize}




==> tex/02_related_work_v1.tex <==
\section{Related Work}
\label{sec:related_work}

Similarly to our work, a number of papers study how to reduce the computational cost of training neural ODEs.
After \cite{chen2018neural} initially presented the neural ODE, \cite{grathwohl2018ffjord} proposed a stochastic estimator of the likelihood to reduce computational cost when using neural ODEs for continuous normalizing flows.
\cite{kelly2020learning,Finlay2020HowTT,pmlr-v139-pal21a} propose additional regularization terms to learn neural ODEs that are easy to integrate.
\cite{ghosh2020steer} propose to regularize the neural ODE by randomly sampling the end time of the ODE during training.
% reduce the stiffness of the learned neural ODE.
\color{red}
Add numerical results of how much we beat them by.
\color{black}

Similarly to our work, \cite{Poli2020HypersolversTF} explicitly study the interplay between the selected numerical integration scheme, and the neural network parametrizing the ODE. 
We note that this work does not present a technique for the training of the neural ODE, but instead they learn to predict the approximation error of a given numerical integrator.
% Although this work does not present a technique for the training of the neural ODE, they also learn to predict the approximation error of the numerical integrator.
By contrast, we propose both a method to train the neural ODE, as well as a method to simplify the learning of the approximation error by taking advantage of regularity assumptions on the system dynamics.
\color{red}
Add numerical results about how much we beat them.
\color{black}
% Finally, we note that while all of the above works rely on Runge-Kutta methods for the numerical integration of the neural ODE, our work proposes a Taylor series method for this purpose.

% We additionally propose a method to efficiently learn the midpoint value of the expansion, in order to simplify the task of learning the approximation error of the numerical integration step.

% However, our work differs from all of the above in that we are the first to use Taylor series methods for the integration of the neural ODE.
Highly accurate Taylor expansion methods for the numerical solution of differential equations have a long history \cite{barton1971automatic,corliss1982solving,kunovsky1994modern,nedialkov2005solving}.
Chapter 13 of \cite{Griewank2000EvaluatingD} discusses the automatic computation of Taylor coefficients, and how these coefficients can be used to solve ODEs.
However, Runge-Kutta methods \cite{Runge1895,Kutta,alexander1990solving,butcher2016numerical} are more frequently used, as they do not require evaluations of the high-order derivatives of the system's vector field.
% However, Taylor series methods are often passed over for algorithms that do not require evaluations of the high-order derivatives of the system's vector field, such as the more frequently used Runge-Kutta methods \cite{Runge1895,Kutta,alexander1990solving,butcher2016numerical}.
% These more common numerical integration schemes are typically what is used to train neural ODEs.
In this work, we demonstrate that owing to existing libraries for efficient automatic differentiation of neural networks, Taylor expansion methods are particularly well suited for the training of neural ODEs.
Our work is the first to apply such Taylor expansion methods in the context of neural ODEs.



==> tex/03_background_v1.tex <==
\section{Solutions of Ordinary Differential Equations (ODEs)}
\label{sec:preliminaries}
In this section, we introduce some necessary background on ordinary differential equations (ODEs), on algorithms for the numerical integration of ODEs, and on neural ODEs.
% a data-driven approach to learn ODEs from data using neural network parameterizations.

Let the  function $\vectorField (\state, \timeval) : \stateSpace \times \mathbb{R}_+ \mapsto \mathbb{R}^\stateDim$ be \emph{Lipschitz-continuous} in $\state$ and $\timeval$. An ordinary differential equation specifies the instantaneous change of a vector-valued signal of time $\dot{\state} : \mathbb{R_+} \mapsto \stateSpace$ via:
\begin{align}
    \dot{\state}(\timeval) = \vectorField(\state(\timeval), \timeval).\label{eq:dynamics-formulation}
\end{align}
The function $\vectorField$ can model, for example, the equations of motion of rigid-body dynamics or the density flow in generative models.
% or even \textcolor{blue}{another example here maybe}.

% \textbf{Initial Value Problems (IVP)}\\
Given some initial state $\state_0 = x(\initTime) \in \stateSpace$ at time $\timeval_0 \geq 0$, we wish to compute a solution to \eqref{eq:dynamics-formulation}.
In this work, we are specifically interested in predicting the value of the state $\state(\timeval)$, at an arbitrary future point in time $\predictionTime \geq \initTime$.
The value of \(\state(\predictionTime)\) can be found by \textit{integrating} or \textit{solving} the ODE: $\state (\predictionTime) = \state(\initTime) + \int_{\initTime}^{\predictionTime} \vectorField (\state (s), s) \,ds.$
% We refer to the process of finding such future state value as \emph{integrating} or \emph{solving} the ODE. 
% We emphasize that it is in general not possible to obtain analytic solutions to ODEs due to potential non-linearities in $\vectorField$.
\subsection{Runge-Kutta Methods for the Numerical Integration of ODEs}
% \textbf{Runge-Kutta Methods for the Numerical Integration of ODEs}\\
Runge-Kutta (RK) methods~\cite{Runge1895,Kutta} are widely used numerical integration techniques for ODEs. Such methods approximate the solutions of the ODEs by first partitioning the time interval $[\initTime, \predictionTime]$ into a series of smaller intervals $[\timeval_i, \timeval_{i+1}]$, where $\timeval_{i} = \initTime + i \timestep$,  $\timeval_H = \predictionTime$, and $\timestep$ denotes the integration step-size. The final state $\state(\predictionTime)$ is obtained by iteratively computing the states at the intermediary time values $\timeval_i$ using \eqref{eq:general_ode_sol_intermediate_steps} and \eqref{eq:general_ode_sol}.
% \begin{align}
%     r_j = \vectorField\Big( \timeval_i + c_j \timestep, \state(t_{i-1}) + \sum\nolimits_{l=1}^j A_{jl} r_l \Big), \; \hat{\state}(\timeval_i) = \state (\timeval_{i-1}) + \timestep \sum\nolimits_{l=1}^p b_l r_l,
% \end{align}
\begin{equation}
    r_j = \vectorField\Big( \timeval_i + c_j \timestep, \state(t_{i-1}) + \sum\nolimits_{l=1}^j A_{jl} r_l \Big)
    \label{eq:general_ode_sol_intermediate_steps}
\end{equation}
\begin{equation}
    \hat{\state}(\timeval_i) = \state (\timeval_{i-1}) + \timestep \sum\nolimits_{l=1}^p b_l r_l
    \label{eq:general_ode_sol}
\end{equation}
% 
Here, $\hat{\state}(\timeval_i)$ is an approximation of the solution at $\timeval_i$, $p$ denotes the order of the RK method, and the coefficients $A \in \mathbb{R}^{p\times p} , b \in \mathbb{R}^p$ and $c \in \mathbb{R}^p$ are tableau coefficients specific to the order $p$. 
Hence, integrating an ODE using a $p^{th}$ order RK method amounts to $\mathcal{O}(p H)$ memory requirements and time complexity, where $H$ denotes the number of time steps used to discretize the interval \([\initTime, \predictionTime]\). 
We refer to fixed-step RK methods as RK methods for which the time step $\timestep$ is fixed. 
On the other hand, adaptive-step RK methods automatically select and refine the values of $\timestep$ during the numerical integration process in order to ensure that the resulting approximation error is sufficiently small. 
% On the other hand, adaptive-step RK methods efficiently choose and refine $\timestep$ at each integration time such that the approximation error is sufficiently small. 
As a result, adaptive-step RK methods do not provide any explicit upper bounds on the amount of memory or the number of functions evaluations required by the method.
The availability of such upper bounds can be critical in applications with real-time requirements \cite{Poli2020HypersolversTF}.
% which is critical in applications with real-time requirements~\cite{Poli2020HypersolversTF}.

\subsection{Taylor Expansion Methods for the Numerical Integration of ODEs}
% \textbf{Taylor Expansion Methods for the Numerical Integration of ODEs}\\
Taylor expansions are a technique used to approximate a function near a particular expansion point using polynomials.
% Taylor expansion is a technique to approximate a function near a particular point with polynomials. 
Similarly to as with RK methods, when using Taylor expansion methods for numerical integration over an interval \([\initTime, \predictionTime]\), we begin by partitioning \([\initTime, \predictionTime]\) into smaller sub-intervals \([t_i, t_{i+1}]\) before iteratively solving sub-problems over each of these sub-intervals.
% computations over these sub-intervals.
% In the context of numerically integrating an ODE over the sub-interval \([t_i, t_{i+1}]\), yields an approximation \(\hat{\state}(\timeval_{i+1})\) of the state at time \(t_{i+1}\), given the value of the state \(\state(t_i)\) at time \(\t_i\).
In the context of numerically integrating an ODE over the sub-interval \([t_i, t_{i+1}]\), \eqref{eq:taylor_ode_solution} yields an approximation \(\hat{\state}(\timeval_{i+1})\) of the state at time \(t_{i+1}\), given the value of the state \(\state(t_i)\) at time \(\timeval_i\).
% In the context of computing the value of $\state(\timeval_{i+1})$ by numerically integrating ~\eqref{eq:dynamics-formulation} given an initial state $\state(\timeval_i)$, a $p^{th}$ order Taylor expansion provides an approximation $\hat{\state}(\timeval_{i+1})$ of $\state(\timeval_{i+1})$ through the equation
% as follows: $\hat{\state}(\timeval_{i+1}) = \state(\timeval_i) + \sum\nolimits_{l=1}^p (\timeval_{i+1}-\timeval_i)^l\vectorField^{[l]}(\state(\timeval_i), \timeval_i)$,
% 
\begin{equation}
    \hat{\state}(\timeval_{i+1}) = \state(\timeval_i) + \sum\nolimits_{l=1}^p \timestep^l\vectorField^{[l]}(\state(\timeval_i), \timeval_i)
    \label{eq:taylor_ode_solution}
\end{equation}
% 
% \begin{align}
%     \hat{\state}(\timeval_{i+1}) = \state(\timeval_i) + \sum\nolimits_{l=1}^p (\timeval_{i+1}-\timeval_i)^l\vectorField^{[l]}(\state(\timeval_i), \timeval_i),
% \end{align}
The Taylor coefficients $\vectorField^{[l]}$ can be defined inductively through the equations: $\vectorField^{[1]} = \vectorField, \; \vectorField^{[l+1]} = \frac{1}{l+1} \frac{\partial \vectorField^{[l]}}{\partial \state} \vectorField$. 
Such Taylor coefficients can be efficiently computed via a generalization of forward-mode automatic differentiation, known as \emph{Taylor mode} \cite{Griewank2000EvaluatingD,Bettencourt2019TaylorModeAD,kelly2020learning}. 
Taylor mode automatic differentiation computes the first $p$ Taylor coefficients $\vectorField^{[1]}, \ldots, \vectorField^{[p]}$ exactly in a single pass, with a time cost of only $\mathcal{O}(p^2)$ or of $\mathcal{O}(p \log p)$, depending on the underlying operations involved \cite{kelly2020learning,Griewank2000EvaluatingD}.
% Taylor mode technique computes in a single pass the first $p$ Taylor coefficients $\vectorField^{[l]}$ exactly with a time cost of only $\mathcal{O}(p^2)$ or $\mathcal{O}(p \log p)$.
% We emphasize that $\hat{\state}(\timeval_{i+1})$ is an approximation of the solution $\state(\timeval_{i+1})$ that depends on the time step and the expansion order $p$. 

One reason that RK methods are favored over Taylor expansion methods for the solving of ODEs, is the high computation cost and memory expense associated with finding the Taylor coefficients, i.e. the higher-order derivatives of $\vectorField$. 
% One of the main reasons RK methods are favored for solving ODEs over Taylor expansion-based methods is due to the computation cost and memory expense associated with finding the Taylor coefficients: Higher-order derivatives of $\vectorField$. 
Indeed, while the local truncation error of both a $p$-order Taylor expansion and a fixed-step $p^{th}$ order RK method is $\|\state(\timeval_{i+1}) - \hat{\state}(\timeval_{i+1})\| \leq c (\timeval_{i+1} - \timeval_{i})^{p+1}$ for some $c > 0$, a fixed-step \(p^{th}\) order RK method only requires \(\mathcal{O}(p)\) function evaluations for a single-step integration, while the Taylor expansion method requires \(\mathcal{O}(p^2)\). 


% Indeed,  it has been shown that the local truncated error of a $p$-order Taylor expansion and a $p$-order RK method is $\|\state(\timeval_{i+1}) - \hat{\state}(\timeval_{i+1})\| \leq c (\timeval_{i+1} - \timeval_{i})^{p+1}$ for some $c > 0$. 
% However, a fixed-step $p$-order RK method only requires at most $p$ function evaluations for a one-step integration while Taylor series methods has a $\mathcal{O}(p^2)$ number of function evaluations.
% However, in term of comuptation time, a fixed-step $p$-order RK method only requires at most $p$ function evaluations for a one-step integration while Taylor series methods has a $\mathcal{O}(p^2)$ number of function evaluations.

% The computational and memory bottleneck of Taylor-based methods to solve ODEs
% We denote by $\mathcal{R}_p = \state(\timeval_{i+1}) - \hat{\state}(\timeval_{i+1})$ such an approximation error.
% \begin{align}
%     \vectorField^{[1]} = \vectorField, \; \vectorField^{[l+1]} = \frac{1}{l+1} \frac{\partial \vectorField^{[l]}}{\partial \state} \vectorField 
% \end{align}
% In the context of solving differential equations, Taylor expansion provides approximate solutions 
% + \frac{(y-a)^{p+1}}{(p+1)!} h^{p+1}(\midpoint)
% Let $h : \mathbb{R} \mapsto \mathbb{R}$ be a sufficiently smooth real-valued function on $\mathbb{R}$. A $p$-order Taylor-Lagrange expansion of $h$ around a point $a \in \mathbb{R}$ is a truncated Taylor expansion of order $p$ that incorporates the expansion error via the mean value theorem as follows:
% \begin{align}
%     h(y) = h(a) + \sum\nolimits_{l=1}^p \frac{(y-a)^l}{l!} h^{(l)}(a) + \frac{(y-a)^{p+1}}{(p+1)!} h^{p+1}(\midpoint).
% \end{align}
% Here, $a$ is the center of the expansion, $h^{(l)}$ denotes the $l$-th derivatives of $h$, and $\gamma$ is the so-called \emph{midpoint value} that must satisfy  $ \midpoint \in [a, y]$.
% In the context of solving differential equations, 

\subsection{Neural ODEs}
% \textbf{Neural ODEs}\\
Neural ODEs use a neural network to parameterize the right hand side of \eqref{eq:dynamics-formulation}.
That is, a neural ODE consists of a neural network \(\vectorField_{\nnParams}\) with parameters \(\nnParams\).
Given an input point \(\state\) from the state space, the output of the neural ODE is the result of integrating the ODE that it parameterizes. 
More specifically, the input point \(\state\) is treated as the state at some initial time \(\initTime\), \(\state(\initTime) \defeq \state\), and the underlying neural network \(\vectorField_{\nnParams}\) is integrated to predict the value of the state at a future point in time \(\predictionTime\).
For notational convenience, we represent the output of the neural ODE as \(\neuralODE_{\nnParams}(\state, \initTime, \predictionTime)\).
Equation \eqref{eq:neural_ODE_output} summarizes the forward evaluation of the neural ODE.

\begin{equation}
    \neuralODE_{\nnParams}(\state, \initTime, \predictionTime) \defeq \state +  \int_{\initTime}^{\predictionTime}\vectorField_{\nnParams}(\state(s), s) ds
    \label{eq:neural_ODE_output}
\end{equation}

Given some loss function \(\loss(\neuralODE_{\nnParams}(\state, \initTime, \predictionTime))\) defined on the output of the neural ODE, the network is trained using gradient descent.
We note that the computation of \(\neuralODE_{\nnParams}(\state, \initTime, \predictionTime)\) relies on the numerical integration of the underlying neural network \(\vectorField_{\nnParams}\).
% To compute the gradient of the loss function \(\frac{d \loss}{d \theta}\), 
\cite{chen2018neural} use the adjoint sensitivity method \cite{pontryagin1987mathematical} to compute the gradient of the loss function \(\frac{d \loss}{d \nnParams}\) without differentiating through the forward pass of the numerical integrator, which would incur a high memory cost and introduce additional numerical error. 

While historically all implementations of neural ODEs have relied on Runge-Kutta integration techniques to numerically solve \eqref{eq:neural_ODE_output}, this work proposes the use of Taylor expansion methods.

% To compute the output of the neural ODE, any numerical integration technique may be used.

% To compute the output of the neural ODE, while any numerical integration technique may be used, prior works have all used Runge-Kutta techniques.


% Neural ODEs model dynamical systems by parameterizing differential equations as neural networks.
% In particular, given an ODE system model as described by \eqref{eq:dynamics-formulation}, the function \(\vectorField\) is parameterized as a neural network with parameters \(\nnParams\).

% Given an ODE system model, as described by \eqref{eq:dynamics-formulation}, neural ODEs use a neural network to parameterize the function \(\vectorField\). 
% That is, a neural ODE trains a neural network \(\vectorField_{\nnParams}\) with parameters \(\nnParams\).

% % \subsection{Neural ODEs}
% % \label{sec:preliminaries_neural_odes}
% Neural ODEs model dynamical systems by parameterizing the governing ordinary differential equations using neural networks.
% More specifically, consider arbitrary non-linear dynamics expressed in terms of the following ordinary differential equation (ODE):
% % 
% \begin{equation}
%     \dot{\state} = \vectorField (\state, \controlInput).
%     % \frac{d \state}{dt} = \vectorField(\state, \controlInput)
%     \label{eq:vector_field_definition_dynamics}
% \end{equation}
% % 
% Here, the state $\state : \mathbb{R}_+ \mapsto \stateSpace$ is a continuous-time signal, the control input  $\controlInput : \mathbb{R}_+ \mapsto \controlSpace$ is a (possibly non-continuous) signal of time, and the vector field $\vectorField : \stateSpace \times \controlSpace \mapsto \mathbb{R}^\stateDim$ is assumed to be unknown and possibly non-linear. 
% Here, $\stateDim$ denotes the dimension of the state. 
% While it is straightforward to explicitly include time dependency in~\eqref{eq:vector_field_definition_dynamics}, we omit it for clarity and for notational simplicity. 

% Neural ODEs parametrize the unknown vector field \(\vectorField\) using a neural network \(\vectorField_{\nnParams}\) with parameters \(\nnParams\).
% The objective of the neural ODE is to be able to predict future state values \(\state_{k+1}, ..., \state_{k + \rollout +1}\), given the current state value \(\state_k\) and a sequence of control inputs \(\controlInput_k, \ldots, \controlInput_{k + \rollout}\).
% The network is then trained using a finite dataset \(\dataset\) of system trajectories -- time-series data of states and control inputs. 
% We write \(\dataset = \{\trajectory_1, \ldots, \trajectory_{|\dataset|}\}\) where \(\trajectory = \{(\state_0, \controlInput_0), (\state_1, \controlInput_1), \ldots, (\state_{\trajectoryTimeHorizon}, \controlInput_{\trajectoryTimeHorizon})\}\) for each \(\trajectory \in \dataset\) and where \(\state_i = \state(t_i)\) denotes the state at time \(t_i\), \(\controlInput_i = \controlInput(t_i)\) denotes the control input at time \(t_i\), and \(t_0 < t_1 < \ldots < t_{\trajectoryTimeHorizon}\) is an increasing sequence of points in time.

% Throughout the paper, we assume that a finite dataset $\dataset$ of system trajectories -- time-series data of states and control inputs -- is available, in lieu of the system's model. 
% That is, we are given a set $\dataset = \{ \trajectory_1, \hdots, \trajectory_{\datasetDim}\}$ of trajectories $\trajectory = \{(\state_0, \controlInput_0), (\state_1, \controlInput_1), \hdots,(\state_{\trajectoryTimeHorizon}, \controlInput_{\trajectoryTimeHorizon})\}$, where $\state_i = \state(t_i)$ is the state at time $t_i$, $\controlInput_i = \controlInput(t_i)$ is the control input applied at time $t_i$, and $t_0 < t_1 < \ldots < t_{\trajectoryTimeHorizon}$ is an increasing sequence of points in time.
% We seek to learn a function to predict future state values $\state_{k+1},\hdots,\state_{k+\rollout+1}$, given the current state value $\state_k$ and a sequence of control inputs $\controlInput_k,\hdots,\controlInput_{k+\rollout}$.

% We propose to parameterize and to learn the unknown vector field $h$, as opposed to learning a prediction function that maps directly from a history of states and control inputs to the predicted next state. 
% This choice to parametrize a model of the vector field is primarily motivated by the two following points: 
% (1) A-priori knowledge derived from physical principles is typically most easily expressed in terms of the system's vector field;
% (2) Recent work~\cite{chen2018neural} has demonstrated that parametrizing the vector field results in models that are able to approximate time-series data with more accuracy than approaches that directly estimate the next state.
% We thus build a framework capable of learning the vector field $h$ from the dataset $\dataset$ of trajectories, while also taking advantage of prior knowledge surrounding the functional form of the vector field.


==> tex/04_taylor_nets_v1.tex <==
\section{Taylor-Lagrange Networks}

In this section, we propose an algorithm for the training of neural ODEs.
As described above, we parameterize the system's vector field \(\vectorField\) using a neural network with parameters \(\nnParams\), and we compute outputs of the neural ODE model by numerically integrating the neural network \(\vectorField_{\nnParams}\) in time.

% We assume that the available training datapoints are tuples of the form \((\initTime, \predictionTime, \state, \trueNextState)\) where \(\initTime\) is an initial time, \(\predictionTime\) is a desired prediction time, and  \(\state\), \(\trueNextState\) are the values of the state at the initial and prediction times respectively. 
% This algorithm numerically integrates the dynamics function \(\vectorField_{\nnParams}\) through direct use of the Taylor-Lagrange expansion of \(\vectorField_{\nnParams}(\state(t))\) in time. 
% More specifically, the algorithm builds a truncated Taylor expansion including terms up to some pre-specified order \(p\).
% The algorithm additionally estimates value of the truncated expansion's approximation error in order to obtain a more accurate numerical integration step.

\subsection{Taylor-Lagrange Numerical Integration of the neural ODE}

\label{sec:TL_numerical_integration_of_neural_ode}

In order to compute a forward pass of the neural ODE \(\neuralODE_{\nnParams}(\state, \initTime, \predictionTime)\), we propose to compute the right hand side of \eqref{eq:neural_ODE_output} via a direct use of the Taylor-Lagrange expansion of \(\vectorField_{\nnParams}(\state(t), t)\) in time.
% We propose to numerically integrate the dynamics function \(\vectorField_{\nnParams}\) via a direct use of the Taylor-Lagrange expansion of \(\vectorField_{\nnParams}(\state(t))\) in time.
Note that we use the term Taylor-Lagrange expansion to refer to the truncated Taylor expansion including the Lagrange form of the remainder.

More specifically, similarly to as described above, the time interval \([\initTime, \predictionTime]\) is broken into a collection of \(\numIntervals\) smaller intervals \([t_i, t_{i+1}]\).
For notational convenience, we assume the value of the integration time step is fixed, i.e. \(\timestep = t_{i+1} - t_{i}\) for all \(i = 0, \ldots, \numIntervals - 1\).
Given the value of the state \(\state(t_{i})\) at time \(t_i\), we compute the value of the next state \(\state(\timeval_{i+1})\) via a \(p^{th}\) order Taylor-Lagrange expansion, which we denote by \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\).
% We denote this estimated value of \(\state(t_{i+1})\) by \(\taylorLagrange_{\nnParams}(\state, \initTime, \predictionTime)\).
The output of the neural ODE \(\neuralODE_{\nnParams}(\state, \initTime, \predictionTime)\) is then computed by iteratively using \(TL_{\nnParams}\) to compute approximations of the integral of \(\vectorField_{\nnParams}\) over the time interval \([\timeval_i, \timeval_{i+1}]\).
Equation \eqref{eq:taylor_lagrange_expansion} details how the value of \(\taylorLagrange_{\nnParams}(\state, t_{i}, t_{i+1})\) is calculated using \(\vectorField_{\nnParams}\).
% 
\begin{equation}
\begin{split}
    \taylorLagrange_{\nnParams}(\state, t_i, t_{i+1}) \defeq \state + \sum\nolimits_{l=1}^{p-1} & \timestep^l \vectorField_{\nnParams}^{[l]}(\state, \timeval_i) \\ 
    & + \timestep^{p} \vectorField_{\nnParams}^{[p]}(\midpoint, \midpointTime)
\end{split}
\label{eq:taylor_lagrange_expansion}
\end{equation}
% 
Here, $\midpoint \in \stateSpace$ is some vector called the \emph{midpoint} whose components are element-wise contained between \(\state(t_i)\) and \(\state(\timeval_{i+1}) = \taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\).
% that must lye between $\state(\timeval_i)$ and $\state(\timeval_{i+1}) = \taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})$. 
If the midpoint were known exactly, then \(\timestep^p \vectorField_{\nnParams}^{[p]}(\midpoint)\) provides the exact value of the approximation error of the expansion.
In other words, if \(\midpoint\) were known, \eqref{eq:taylor_lagrange_expansion} provides an exact expression for the integral \(\state(t_i) + \int_{t_i}^{t_{i+1}} \vectorField_{\nnParams}(\state(s), s) ds\).
% If such a midpoint value is known, then it straightforwardly provides the exact approximation error of a truncated $(p-1)$-order Taylor expansion through computing the highest order Taylor coefficient. 

% Besides, the midpoint value is a function of the state $\state(\timeval_i)$, the time step $\timeval_{i+1}-\timeval_{i}$, and it can be as complex as the function $\vectorField_\nnParams$ itself.

% The values of the state \(\state(t_{i+1})\) at time \(t_{i+1}\) are iteratively calculated from the value of the state at the prior integration time step \(\state(t_{i})\) via the Taylor-Lagrange expansion of \(\vectorField_{\nnParams}\).


% This algorithm numerically integrates the dynamics function \(\vectorField_{\nnParams}\) through direct use of the Taylor-Lagrange expansion of \(\vectorField_{\nnParams}(\state(t))\) in time. 
% More specifically, the algorithm builds a truncated Taylor expansion including terms up to some pre-specified order \(p\), while also using estimates of the value of the expansion's approximation error to obtain a more accurate numerical integration step.
% \Eqref{eq:taylor_lagrange_expansion} summarizes 

% That is, instead of using the truncated Taylor expansion given in \eqref{eq:taylor_ode_solution} to integrate the neural network \(\vectorField_{\nnParams}\), we additionally include the term
% That is, instead of using the truncated form of the Taylor expansion provided in \eqref{eq:taylor_ode_solution}, and propagating the expansion error during training, we propose to learn the exact solution of the ODE given by the so-called $p^{th}$ order Taylor-Lagrange expansion:
% \begin{equation}
%     \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}) \defeq \state (\timeval_i) + \sum\nolimits_{l=1}^{p-1} (\timeval_{i+1}-\timeval_i)^l \vectorField_{\nnParams}^{[l]}(\state(\timeval_i), \timeval_i) + (\timeval_{i+1}-\timeval_{i})^{p} \vectorField_{\nnParams}^{[p]}(\midpoint),
% \end{equation}
% for some value $\midpoint$ called \emph{midpoint} value that must lye between $\state(\timeval_i)$ and $\state(\timeval_{i+1}) = \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1})$. If such a midpoint value is known, then it straightforwardly provides the exact approximation error of a truncated $(p-1)$-order Taylor expansion through computing the highest order Taylor coefficient. Besides, the midpoint value is a function of the state $\state(\timeval_i)$, the time step $\timeval_{i+1}-\timeval_{i}$, and it can be as complex as the function $\vectorField_\nnParams$ itself.

% \textcolor{blue}{Maybe an example of a first order Taylor Lagrange expansion here to ease reading and show how the Taylor coefficient of order 1 is computed ?}

\subsection{Learning to Predict the Midpoint Value}
\label{sec:learning_the_midtpoint}

While no closed form expression for \(\midpoint\) exists, we propose to learn to predict its value given the state \(\state\) and the time step \(\timestep\).
However, learning to predict the midpoint directly is a challenging problem in general.
% In particular, without putting any restrictions on the predicted values of \(\midpoint\), 
We instead propose to use the result of Theorem \ref{thm:expression-midpoint}, which provides a closed-form expression for the midpoint in terms of some unknown term \(\midpointUnknownTerm \in \stateSpace\), to simplify the task of learning to predict \(\midpoint\).

\begin{theorem}[Simplified Midpoint Expression]\label{thm:expression-midpoint}
    If $\vectorField_{\nnParams}$ is a Lipschitz-continuous function, then the midpoint value $\midpoint$ of the Taylor-Lagrange expansion \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\) satisfies
    \begin{equation}
        \midpoint = \state + \midpointUnknownTerm(\state, \timestep) \odot  \vectorField_{\nnParams}(\state, \timeval_i), \text{ and, } \label{eq:midpoint-simple}
    \end{equation}
    \begin{equation}
        \min \{\state, \taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1}) \} \leq \midpoint \leq \max \{\state,  \taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\},\label{eq:midpoint-constr}
    \end{equation}
    % \begin{align}
    %     &\midpoint = \state(\timeval_i) + \midpointUnknownTerm(\state(\timeval_i), \timestep) \odot  \vectorField_{\nnParams}(\state(\timeval_i), \timeval_i), \label{eq:midpoint-simple}\\
    %     &\min \{ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}), \state(\timeval_{i}) \} \leq \midpoint_\nnParams(\state(\timeval_i), \timeval_{i+1}-\timeval_{i}) \leq \max \{ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}), \state(\timeval_{i}) \},\label{eq:midpoint-constr}
    % \end{align}
    where $\midpointUnknownTerm$ is some function mapping from the state \(\state\) and time step \(\timestep\) to \(\stateSpace\), \(\odot\) denotes the element-wise multiplication operation, and the \(\min\) and \(\max\) operators are applied element-wise.
\end{theorem}

% simplifies the problem of learning a function predicting the midpoint by

% To do so, we parameterize a neural network \(\midpoint_{\nnParamsMidpoint}\) that takes the values of \(\state\) and \(\timestep\) as input.

% To learn the midpoint value \(\midpoint\) of a particular Taylor-Lagrange expansion \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\), we parameterize a neural network \(\midpoint_{\nnParamsMidpoint}\) that takes the \(\state\) and the time step \(t_{i+1} - t_{i}\) as input, and predicts the value of \(\midpoint\).

% \paragraph{Simplify the Midpoint Learning.} 
% In this paper, we propose to learn the vector field $\vectorField_{\nnParams}$ alongside the midpoint value. To this end, we parameterize the midpoint value by a neural network having as inputs the state and the time step. We denote by $\midpoint_{\nnParams}$ the resulting function, and  we consider that the parameter $\nnParams$ contains both the parameters of the vectorfield $\vectorField$ and the midpoint $\midpoint$ parameterizations. To cope with the complexity of learning such a midpoint, we provide, in Theorem \ref{thm:expression-midpoint} a closed-form expression aiming at simplify its learning by reusing the knowledge of the vector field $\vectorField_{\nnParams}$.

% \begin{theorem}[Simplified Midpoint Learning]\label{thm:expression-midpoint}
%     If $\vectorField_{\nnParams}$ is a Lipschitz-continuous function, then the midpoint value $\midpoint(\nnParams)$ evaluated at $\state(\timeval_i)$ to predict $ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1})$ satisfies the following:
%     \begin{align}
%         &\midpoint_\nnParams(\state(\timeval_i), \timeval_{i+1}-\timeval_{i}) = \state(\timeval_i) + \midpoint^1_\nnParams(\state(\timeval_i), \timeval_{i+1}-\timeval_{i}) \vectorField_{\nnParams}(\state(\timeval_i), \timeval_i), \label{eq:midpoint-simple}\\
%         &\min \{ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}), \state(\timeval_{i}) \} \leq \midpoint_\nnParams(\state(\timeval_i), \timeval_{i+1}-\timeval_{i}) \leq \max \{ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}), \state(\timeval_{i}) \},\label{eq:midpoint-constr}
%     \end{align}
%     where $\midpoint_\nnParams^1$ is the actual neural network that will be trained to predict the midpoint value through~\eqref{eq:midpoint-simple}, and the constraint in~\eqref{eq:midpoint-constr} ensures that the midpoint value lies between the current and next state values.
% \end{theorem}


% We provide a proof of Theorem~\ref{thm:expression-midpoint} in Appendix~\ref{}. Specifically, the theorem is obtained by using tools from interval Taylor-based reachability analysis. The formulation in~\eqref{eq:midpoint-simple} is derived from our explicit formula for the so-called \emph{apriori} enclosure: A set guaranteed to contain the next state value $\neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1})$ under some local Lipschitz bound knowledge. 

Theorem~\ref{thm:expression-midpoint} is obtained using tools from interval Taylor-Langrange based reachability analysis \cite{djeumou2021fly}.
More specifically, the equation given in \eqref{eq:midpoint-simple} is derived from explicit formulas for the so-called \emph{apriori} enclosure -- a set derived from the local Lipschitzness of \(\vectorField_{\nnParams}\) that is guaranteed to contain the value of \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\).
The constraint in~\eqref{eq:midpoint-constr} ensures that the midpoint lies between the center point and the evaluation point of the Taylor-Lagrange expansion.
A proof of Theorem~\ref{thm:expression-midpoint} is provided in the Appendix.

% \color{red}
% Besides, a stronger result in the proof of Theorem~\ref{thm:expression-midpoint} suggests that the resulting neural network $\midpoint^1_\nnParams$ is a function of only the Lipschitz bounds of $\vectorField_\nnParams$, the time step $\timeval_{i+1}- \timeval_{i}$, and a small value between $-1$ and 1 that depends on $\state(\timeval_i)$. Hence, the claim that \eqref{eq:midpoint-simple} is a simpler learning representation for the midpoint value.
% \color{black}

Given the result of Theorem \ref{thm:expression-midpoint}, we propose to parameterize the unknown function \(\midpointUnknownTerm_{\nnParamsMidpoint}\) using a neural network with parameters \(\nnParamsMidpoint\).
For notational simplicity, we use \(\midpoint_{\nnParamsMidpoint}(\state, \timeval_i, \timestep)\) to denote the value of the right hand side of \eqref{eq:midpoint-simple} when \(\midpointUnknownTerm\) is approximated by \(\midpointUnknownTerm_{\nnParamsMidpoint}\).
Given the predicted midpoint value \(\midpoint_{\nnParamsMidpoint}(\state, \timeval_i, \timestep)\) of the \(p^{th}\) order Taylor-Lagrange expansion \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\), we estimate the expansion's approximation error as \(\timestep^{p}\vectorField_{\nnParams}^{[p]}(\midpoint_{\nnParamsMidpoint}(\state, \timeval_i, \timestep))\).
% when computing the right hand side of \eqref{eq:taylor_lagrange_expansion}.

\input{algs/evaluation_alg}

\subsection{Bounding the Error of the Taylor-Lagrange Integrator}
% \paragraph{Accuracy of Taylor-Lagrange with Learned Midpoint.}
We seek to bound the error on a \(p^{th}\) order Taylor-Lagrange expansion which uses a learned midpoint value predictor \(\midpoint_{\nnParamsMidpoint}\).
Such an error bounds straightforwardly depends on how well \(\midpoint_{\nnParamsMidpoint}\) approximates the true midpoint \(\midpoint\), as described in Theorem \ref{thm-approximation-error}.
% We seek to provide an approximation error bound on a $p^{th}$ order Taylor-Lagrange expansion with learned midpoint value $\midpoint_{\nnParams}$. Such error straightforwardly depends on how well $\midpoint_{\nnParams}$, defined in~\eqref{eq:midpoint-simple}, can approximate the midpoint $\midpoint$. 
A proof of Theorem~\ref{thm-approximation-error} is provided in the Appendix.

\begin{theorem}[Integration Accuracy]\label{thm-approximation-error}
    If the learned midpoint predictor \(\midpoint_{\nnParamsMidpoint}\) is a $\mathcal{O}(\eta)$ approximator to the midpoint value $\midpoint$ of the Taylor-Lagrange expansion of \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\), then $\| \state(\timeval_{i+1}) - \taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1}) \| \leq c \eta \timestep^{p+1}$ for some $c > 0$ that depends on the Lipschitz constant of $\vectorField_{\nnParams}$.
\end{theorem}   

% \begin{theorem}[Integration Accuracy]\label{thm-approximation-error}
%     If the trained neural network $\midpoint_{\nnParams}$ given in~\eqref{eq:midpoint-simple} is a $\mathcal{O}(\eta)$ approximator of the unknown midpoint value $\midpoint$ of the Taylor-Lagrange expansion of $\vectorField_{\nnParams}$, then the local truncation error is $\mathcal{O}((\timeval_{i+1}-\timeval_{i})^{p+1} \eta)$, i.e., $\| \state(\timeval_{i+1}) - \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}) \| \leq c \eta (\timeval_{i+1}-\timeval_{i})^{p+1}$ for some real positve value $c$ that depends on the Lipschitzness of $\vectorField_{\nnParams}$.
% \end{theorem}   


%%%%%%%%%%%%%%%%%%%%%
% We note that trying to use \(\midpoint_{\nnParamsMidpoint}(\state, \timeval_i, \timestep)\) to compute \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\) results in a circular dependency; the value of \(\midpoint_{\nnParamsMidpoint}\) relies on the value of \(\taylorLagrange_{\nnParams}\), however, \(\midpoint_{\nnParamsMidpoint}\) is simultaneously being used to compute the value of \(\taylorLagrange_{\nnParams}\).
% In order to get around this issue and to properly use the estimated approximation error \(\midpoint_{\nnParamsMidpoint}\) to compute \(\taylorLagrange_{\nnParams}\), we proceed as follows.
% We first compute \(\taylor_{\nnParams}(\state, \timeval_i, \timeval_{i+1}) = \state + \sum_{i=1}^{p-1} \timestep^{l} \vectorField_{\nnParams}^{[l]}(\state, \timeval_i)\), i.e. the truncated Taylor expansion of \(\vectorField_{\nnParams}\) without the approximation error term.
% We then compute the value of \(\midpoint_{\nnParamsMidpoint}(\state, \timeval_i, \timestep)\) while using \(\taylor_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\) instead of \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\) to define the inequality constraints in \eqref{eq:midpoint-constr}.
% Finally, we substitute \(\midpoint_{\nnParamsMidpoint}(\state, \timeval_i, \timestep)\) into \eqref{eq:taylor_lagrange_expansion} to compute the value of \(\taylorLagrange_{\nnParams}(\state, \timeval, \timeval_{i+1})\).
%%%%%%%%%%%%%%%%%%%%%%%

% Intuitively, consider a one dimensional ODE and assume for the sake of the illustration that $\timeval_{i+1} - \timeval_{i}$ is sufficiently small such that $\state(\timeval_{i+1}) = \state(\timeval_i) + (\timeval_{i+1} - \timeval_{i}) \vectorField_{\nnParams}(\state(\timeval_i), \timeval_i)$ is a good approximation of the next state value. Then, a simple and expressive parameterization of the midpoint that uses the knowledge of the vector field is given by $\state(\timeval_i) + \alpha \vectorField_{\nnParams}(\state(\timeval_i), \timeval_i)$, for some real number $\alpha = \midpoint^1$.

% \textcolor{blue}{Some details about the loop issue on the constraint here and the fact that in scenario where the data are directly over state values, we can have explicit (non-dependent on the unknown next state) constraints (7)}

\subsection{Training the Taylor-Lagrange Networks}

Using the methods described in \S \ref{sec:TL_numerical_integration_of_neural_ode} and \S \ref{sec:learning_the_midtpoint}, we compute the output of the neural ODE \(\neuralODE_{\nnParams}(\state, \initTime, \predictionTime)\) by iteratively using \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\) to numerically integrate \(\vectorField_{\nnParams}\) over the time intervals \([t_i, t_{i+1}]\).
Given a dataset \(\dataset = \{(\state^j, \initTime^j, \predictionTime^j, \trueNextState^j)\}_{j=1}^{|\dataset|}\), where each datapoint consists of an initial state \(\state^j\), an initial time \(\initTime^j\), a prediction time \(\predictionTime^j\), and the value of the state at the prediction time \(\trueNextState^j\), we simultaneously train \(\nnParams\) and \(\nnParamsMidpoint\) via the optimization problem given in \eqref{eq:loss_opt_problem}.

\begin{equation}
\begin{split}
    \min_{\nnParams, \nnParamsMidpoint}  & \sum_{(\state^j, \initTime^j, \predictionTime^j, \trueNextState^j) \in \dataset} \left[
    \loss(\neuralODE_{\nnParams}(\state^j, \initTime^j, \predictionTime^j), \trueNextState^j) \right. \\
    & \left. + \penaltyCoef * \penaltyTerm(\state^j, \initTime^j, \predictionTime^j) + \regularizationCoef * \regTerm(\state^j, \initTime^j, \predictionTime^j)
    \right]
\end{split}   
\label{eq:loss_opt_problem}
\end{equation}

Here, \(\loss(\neuralODE_{\nnParams}(\state, \initTime, \predictionTime))\) is some loss function defined on the outputs of the neural ODE, and \(\penaltyCoef, \regularizationCoef \geq 0\) are scalar parameters.
\(\penaltyTerm(\state, \initTime, \predictionTime)\) is a function measuring of the extent to which the constraints in \eqref{eq:midpoint-constr} are violated throughout the numerical integration of \(\vectorField_{\nnParams}\) from \(\initTime\) to \(\predictionTime\).
We note that the inclusion of \(\penaltyTerm\) in \eqref{eq:loss_opt_problem} penalizes the optimization objective if the neural network \(\midpoint_{\nnParamsMidpoint}\) learns to outputs midpoint values that are infeasible; the midpoint should always take values between the expansion point and the evaluation point of the Taylor series.
% 
% This constraint helps to prevent the model from learning far away points thus inflating the error term in order to overfit the training data.
% \(\penaltyCoef, \regularizationCoef \geq 0\) are scalar parameters.
\begin{equation}
\begin{split}
    \penaltyTerm(\state, & \initTime, \predictionTime) = \sum_{i=0}^{\numIntervals} \Bigl[ l_{hinge} \Bigl( \midpoint_{\nnParamsMidpoint}(\hat{\state}_i, \timeval_i, \timestep) \Bigr. \Bigr. \\
    & \quad \quad \quad \quad \quad \quad \quad \Bigl. - \max\{\hat{\state}_i, \taylorLagrange_{\nnParams}(\hat{\state}_i, \timeval_i, \timeval_{i+1})\} \Bigr)^2 \\
    & + l_{hinge} \Bigl( \min\{\hat{\state}_i, \taylorLagrange_{\nnParams}(\hat{\state}_i, \timeval_i, \timeval_{i+1})\} \Bigr.\\
    & \quad \quad \quad \quad \quad \quad \quad \quad \quad \Bigl. \Bigl. - \midpoint_{\nnParamsMidpoint}(\hat{\state}_i, \timeval_i, \timestep)\Bigr)^2 \Bigr]
\end{split}
\label{eq:penaltyTerm}
\end{equation}
% 
Meanwhile, \(\regTerm(\state, \initTime, \predictionTime)\) measures the magnitude of the approximation errors accumulated during numerical integration.
Intuitively, this penalty term ensures that the predicted approximation error values will remain small, preventing the neural network \(\midpoint_{\nnParamsMidpoint}\) from overfitting the training data.
% which is helpful to prevent the neural ODE from using \(\midpoint_{\nnParamsMidpoint}\) from overfitting the training data.
% of the numerical estimator to be as small as possible.
% 
\begin{equation}
    \regTerm(\state, \initTime, \predictionTime) = \sum_{i=0}^{\numIntervals - 1} || \timestep^p \vectorField_{\nnParams}^{[p]}(\midpoint_{\nnParamsMidpoint}(\hat{\state}_i, \timeval_i, \timestep)) ||_2^2
    \label{eq:reg_term}
\end{equation}
% 
In both of the above equations, \(\hat{\state}_i\) denotes integrator-estimated intermediate state value at time \(t_i\).
% The inclusion of this penalty term helps constrain the model of \(\midpoint_{\nnParamsMidpoint}\), preventing it from learning unreasonable values in order to overfit the training data by controlling the 

% \textbf{Regularizing the Approximation Error}\\

% \textcolor{blue}{In order to avoid overfitting (need to explain), we seek for solutoons for which the remainder $(\timeval_{i+1}-\timeval_{i})^{p} \vectorField_{\nnParams}^{[p]}(\midpoint)$ is small. So we penalize.}

% \paragraph{How to Train Neural ODEs using Taylor-Lagrange.}
% 
% \textcolor{blue}{Details on the training algorithms (maybe the algorithm itself)}


% \textcolor{blue}{A table summarizing the number of function evaluation and accuracy of p-order RK, p-order truncated, and p-order Tayla}

% \textcolor{blue}{Some notation needs to be defined: Lipschitz-continuous, sufficiently-smooth, Big $\mathcal{O}$ symbols etc...}


\input{algs/training_alg}

==> tex/04_taylor_nets_v2.tex <==
\section{Taylor-Lagrange Neural Ordinary Differential Equations}

In this section, we propose a methodology for the efficient and accurate training and evaluation of NODEs.
As described in \S \ref{sec:neural_odes}, we parameterize the system's vector field \(\vectorField(\cdot)\) using a neural network \(\vectorField_{\nnParams}(\cdot)\) with parameters \(\nnParams\), and we compute the outputs of the NODE by numerically integrating \(\vectorField_{\nnParams}\) in time.

% We assume that the available training datapoints are tuples of the form \((\initTime, \predictionTime, \state, \trueNextState)\) where \(\initTime\) is an initial time, \(\predictionTime\) is a desired prediction time, and  \(\state\), \(\trueNextState\) are the values of the state at the initial and prediction times respectively. 
% This algorithm numerically integrates the dynamics function \(\vectorField_{\nnParams}\) through direct use of the Taylor-Lagrange expansion of \(\vectorField_{\nnParams}(\state(t))\) in time. 
% More specifically, the algorithm builds a truncated Taylor expansion including terms up to some pre-specified order \(p\).
% The algorithm additionally estimates value of the truncated expansion's approximation error in order to obtain a more accurate numerical integration step.

\subsection{Data-Driven Taylor-Lagrange Numerical Integration of the NODE}

\label{sec:TL_numerical_integration_of_neural_ode}

In order to compute a forward evaluation of the neural ODE, we propose an algorithm that makes direct use of the Taylor-Lagrange expansion of \(\state_{t}\) in time.
Note that we use the term Taylor-Lagrange expansion to refer to the truncated Taylor expansion including the Lagrange form of the remainder.

\paragraph{Partitioning the prediction interval.}
We begin by partitioning the prediction interval \([\initTime, \predictionTime]\) into a collection of \(\numIntervals\) sub-intervals \([t_i, t_{i+1}]\) before iteratively solving sub-problems over each of these sub-intervals.
% Similarly to as with RK methods, when using Taylor expansion methods for numerical integration over an interval \([\initTime, \predictionTime]\), we begin by partitioning \([\initTime, \predictionTime]\) into a collection of \(\numIntervals\) sub-intervals \([t_i, t_{i+1}]\) before iteratively solving sub-problems over each of these sub-intervals.
For notational convenience, we assume the value of the integration time step is fixed, i.e. \(\timestep = t_{i+1} - t_{i}\) for all \(i = 0, \ldots, \numIntervals - 1\).
Given the value of the state \(\state_{t_{i}}\) at time \(t_i\), we compute an approximation of the value of the state at the next time step \(\hat{\state}_{t_{i+1}}\) via a \(p^{th}\) order Taylor-Lagrange expansion of \(\state_{t}\) about time \(\timeval_{i}\), which we denote by \(\taylorLagrange^{\timestep}_{\nnParams}(\state_{\timeval_i}, \timeval_i)\).
% We denote this estimated value of \(\state(t_{i+1})\) by \(\taylorLagrange_{\nnParams}(\state, \initTime, \predictionTime)\).
The output \(\neuralODE_{\nnParams}(\initState, \initTime, \predictionTime)\) of the neural ODE is then computed by iteratively using \(\taylorLagrange^{\timestep}_{\nnParams}(\cdot)\) to compute approximations of the integral of \(\vectorField_{\nnParams}(\cdot)\) over the time interval \([\timeval_i, \timeval_{i+1}]\).
% Equation \eqref{eq:taylor_lagrange_expansion} details how the value of \(\taylorLagrange_{\nnParams}(\state, t_{i}, t_{i+1})\) is calculated using \(\vectorField_{\nnParams}\).

\paragraph{Expressing \(\boldsymbol{\taylorLagrange^{\timestep}_{\nnParams}(\cdot)}\) in Terms of \(\boldsymbol{\vectorField_{\nnParams}(\cdot)}\).}
Note that because \(\vectorField_{\nnParams}(\state)\) estimates the time derivative of the system state \(\state\), the Taylor-Lagrange expansion of \(\state_{t}\) may be expressed in terms of the \textit{Taylor coefficients} \(\vectorField_{\nnParams}^{[l]}(\state)\), which are recursively defined through the equations \(\vectorField^{[1]}_{\nnParams}(\state) = \vectorField_{\nnParams}(\state)\) and \(\vectorField^{[l+1]}_{\nnParams}(\state) = \frac{1}{l+1} [\frac{\partial \vectorField^{[l]}_{\nnParams}}{\partial \state} \vectorField_{\nnParams}](\state)\). 
Equation \eqref{eq:taylor_lagrange_expansion} accordingly presents the Taylor-Lagrange expansion of \(\state_{\timeval}\) about the point in time \(\timeval_{i}\), evaluated at the future time \(\timeval_{i+1} = \timeval_{i} + \timestep\).
% 
\begin{equation}
\begin{split}
    \taylorLagrange_{\nnParams}^{\timestep}(\state_{\timeval_i}) \defeq \state_{\timeval_i} + \sum\nolimits_{l=1}^{p-1} & \timestep^l \vectorField_{\nnParams}^{[l]}(\state_{\timeval_i}) + \hat{R}(\vectorField_{\nnParams}, \state_{\timeval_i}, \timestep)
    % \timestep^{p} \vectorField_{\nnParams}^{[p]}(\midpoint)
\end{split}
\label{eq:taylor_lagrange_expansion}
\end{equation}
% 
The first two terms on the right hand side of \eqref{eq:taylor_lagrange_expansion} make up the \textit{truncated} Taylor expansion of \(\state_{\timeval}\), while \(\hat{R}(\vectorField_{\nnParams}, \state_{\timeval_i}, \timestep)\) is an estimate of the \textit{remainder} of this truncated expansion.
More specifically, \(\hat{R}(\vectorField_{\nnParams}, \state_{\timeval_i}, \timestep)\) should be an estimate of the approximation error of the \(p^{th}\) order expansion; if could estimate this value exactly, \eqref{eq:taylor_lagrange_expansion} would provide an exact evaluation of the integral \(\state_{t_i} + \int_{t_i}^{t_{i+1}} \vectorField_{\nnParams}(\state_{s}) ds\).

% Here, we refer to the values \((\midpoint, \midpointTime)\) collectively as the \textit{midpoint}. 
% The value of \(\midpointTime\) corresponds to some point in time such that \(\timeval_{i} \leq \midpointTime \leq \timeval_{i+1}\).
% Meanwhile, \(\midpoint \defeq \state(\midpointTime) \in \stateSpace\) is defined as the system's state at this midpoint time \(\midpointTime\), given that the system follows the dynamics defined by \(\vectorField_{\nnParams}(\cdot)\) from initial state \(\state(\timeval_i)\).
% If the midpoint were known exactly, then \(\timestep^p \vectorField_{\nnParams}^{[p]}(\midpoint)\) provides the exact value of the approximation error of the expansion.
% In other words, if \(\midpoint, \midpointTime\) were known, \eqref{eq:taylor_lagrange_expansion} provides an exact expression for the integral \(\state(t_i) + \int_{t_i}^{t_{i+1}} \vectorField_{\nnParams}(\state(s)) ds\).

\paragraph{Efficient Computation of the Taylor Coefficients.}
% The Taylor coefficients \(\vectorField^{[l]}_{\nnParams}\) can be defined inductively through the equations \(\vectorField^{[1]}_{\nnParams}(\state) = \vectorField_{\nnParams}(\state)\) and \(\vectorField^{[l+1]}_{\nnParams}(\state) = \frac{1}{l+1} [\frac{\partial \vectorField^{[l]}_{\nnParams}}{\partial \state} \vectorField_{\nnParams}](\state)\). 
The Taylor coefficients \(\vectorField_{\nnParams}^{[1]}(\state), \ldots, \vectorField_{\nnParams}^{[p]}\) can in principle be evaluated using repeated application of forward-mode automatic differentiation to iteratively compute the Jacobian-vector products \([\frac{\partial \vectorField^{[l]}_{\nnParams}}{\partial x} \vectorField_{\nnParams}](\state)\). 
However, doing so would incur a time cost of \(\mathcal{O}(exp(\expansionOrder))\).
We instead use \textit{Taylor mode} automatic differentiation, which computes the first \(\expansionOrder\) Taylor coefficients \(\vectorField^{[1]}_{\nnParams}, \ldots, \vectorField^{[p]}_{\nnParams}\) in a single pass, with a time cost of only $\mathcal{O}(p^2)$ or of $\mathcal{O}(p \log p)$, depending on the underlying operations involved \cite{Griewank2000EvaluatingD,Bettencourt2019TaylorModeAD,kelly2020learning}.

% Such Taylor coefficients can be efficiently computed via a generalization of forward-mode automatic differentiation, known as \emph{Taylor mode} automatic differentiation \cite{Griewank2000EvaluatingD,Bettencourt2019TaylorModeAD,kelly2020learning}. 
% Taylor mode automatic differentiation computes the first $p$ Taylor coefficients $\vectorField^{[1]}, \ldots, \vectorField^{[p]}$ exactly in a single pass, with a time cost of only $\mathcal{O}(p^2)$ or of $\mathcal{O}(p \log p)$, depending on the underlying operations involved \cite{kelly2020learning,Griewank2000EvaluatingD}.

One reason that RK methods are favored over Taylor expansion methods for the solving of ODEs, is the high computation cost and memory expense associated with finding the Taylor coefficients, i.e. the higher-order derivatives of $\vectorField$. 
Indeed, while the local truncation error of both a $p$-order Taylor expansion and a fixed-step $p^{th}$ order RK method is $\|\state(\timeval_{i+1}) - \hat{\state}(\timeval_{i+1})\| \leq c (\timeval_{i+1} - \timeval_{i})^{p+1}$ for some $c > 0$, a fixed-step \(p^{th}\) order RK method only requires \(\mathcal{O}(p)\) function evaluations for a single-step integration, while the Taylor expansion method requires \(\mathcal{O}(p^2)\) in general.

% More specifically, similarly to as described above, the time interval \([\initTime, \predictionTime]\) is broken into a collection of \(\numIntervals\) smaller intervals \([t_i, t_{i+1}]\).
% For notational convenience, we assume the value of the integration time step is fixed, i.e. \(\timestep = t_{i+1} - t_{i}\) for all \(i = 0, \ldots, \numIntervals - 1\).
% Given the value of the state \(\state(t_{i})\) at time \(t_i\), we compute the value of the next state \(\state(\timeval_{i+1})\) via a \(p^{th}\) order Taylor-Lagrange expansion, which we denote by \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\).
% % We denote this estimated value of \(\state(t_{i+1})\) by \(\taylorLagrange_{\nnParams}(\state, \initTime, \predictionTime)\).
% The output of the neural ODE \(\neuralODE_{\nnParams}(\state, \initTime, \predictionTime)\) is then computed by iteratively using \(TL_{\nnParams}\) to compute approximations of the integral of \(\vectorField_{\nnParams}\) over the time interval \([\timeval_i, \timeval_{i+1}]\).
% Equation \eqref{eq:taylor_lagrange_expansion} details how the value of \(\taylorLagrange_{\nnParams}(\state, t_{i}, t_{i+1})\) is calculated using \(\vectorField_{\nnParams}\).
% % 
% \begin{equation}
% \begin{split}
%     \taylorLagrange_{\nnParams}(\state, t_i, t_{i+1}) \defeq \state + \sum\nolimits_{l=1}^{p-1} & \timestep^l \vectorField_{\nnParams}^{[l]}(\state, \timeval_i) \\ 
%     & + \timestep^{p} \vectorField_{\nnParams}^{[p]}(\midpoint, \midpointTime)
% \end{split}
% \label{eq:taylor_lagrange_expansion}
% \end{equation}
% % 
% Here, $\midpoint \in \stateSpace$ is some vector called the \emph{midpoint} whose components are element-wise contained between \(\state(t_i)\) and \(\state(\timeval_{i+1}) = \taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\).
% % that must lye between $\state(\timeval_i)$ and $\state(\timeval_{i+1}) = \taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})$. 
% If the midpoint were known exactly, then \(\timestep^p \vectorField_{\nnParams}^{[p]}(\midpoint)\) provides the exact value of the approximation error of the expansion.
% In other words, if \(\midpoint\) were known, \eqref{eq:taylor_lagrange_expansion} provides an exact expression for the integral \(\state(t_i) + \int_{t_i}^{t_{i+1}} \vectorField_{\nnParams}(\state(s), s) ds\).
% % If such a midpoint value is known, then it straightforwardly provides the exact approximation error of a truncated $(p-1)$-order Taylor expansion through computing the highest order Taylor coefficient. 

% % Besides, the midpoint value is a function of the state $\state(\timeval_i)$, the time step $\timeval_{i+1}-\timeval_{i}$, and it can be as complex as the function $\vectorField_\nnParams$ itself.

% % The values of the state \(\state(t_{i+1})\) at time \(t_{i+1}\) are iteratively calculated from the value of the state at the prior integration time step \(\state(t_{i})\) via the Taylor-Lagrange expansion of \(\vectorField_{\nnParams}\).


% This algorithm numerically integrates the dynamics function \(\vectorField_{\nnParams}\) through direct use of the Taylor-Lagrange expansion of \(\vectorField_{\nnParams}(\state(t))\) in time. 
% More specifically, the algorithm builds a truncated Taylor expansion including terms up to some pre-specified order \(p\), while also using estimates of the value of the expansion's approximation error to obtain a more accurate numerical integration step.
% \Eqref{eq:taylor_lagrange_expansion} summarizes 

% That is, instead of using the truncated Taylor expansion given in \eqref{eq:taylor_ode_solution} to integrate the neural network \(\vectorField_{\nnParams}\), we additionally include the term
% That is, instead of using the truncated form of the Taylor expansion provided in \eqref{eq:taylor_ode_solution}, and propagating the expansion error during training, we propose to learn the exact solution of the ODE given by the so-called $p^{th}$ order Taylor-Lagrange expansion:
% \begin{equation}
%     \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}) \defeq \state (\timeval_i) + \sum\nolimits_{l=1}^{p-1} (\timeval_{i+1}-\timeval_i)^l \vectorField_{\nnParams}^{[l]}(\state(\timeval_i), \timeval_i) + (\timeval_{i+1}-\timeval_{i})^{p} \vectorField_{\nnParams}^{[p]}(\midpoint),
% \end{equation}
% for some value $\midpoint$ called \emph{midpoint} value that must lye between $\state(\timeval_i)$ and $\state(\timeval_{i+1}) = \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1})$. If such a midpoint value is known, then it straightforwardly provides the exact approximation error of a truncated $(p-1)$-order Taylor expansion through computing the highest order Taylor coefficient. Besides, the midpoint value is a function of the state $\state(\timeval_i)$, the time step $\timeval_{i+1}-\timeval_{i}$, and it can be as complex as the function $\vectorField_\nnParams$ itself.

% \textcolor{blue}{Maybe an example of a first order Taylor Lagrange expansion here to ease reading and show how the Taylor coefficient of order 1 is computed ?}

\subsection{Learning to Predict the Midpoint Value}
\label{sec:learning_the_midtpoint}

We refer to \(\midpoint \in \stateSpace\) as the \textit{midpoint} of the Taylor-Lagrange expansion. 
The first two terms on the right hand side of \eqref{eq:taylor_lagrange_expansion} make up the \textit{truncated} Taylor expansion of \(\state_{\timeval}\), while the final term involving \(\midpoint\) is the \textit{remainder} of this truncated expansion.
More specifically, there exists some point in time \(\midpointTime\) with \(\timeval_{i} \leq \midpointTime \leq \timeval_{i+1}\) such that when we define \(\midpoint \defeq \state_{\midpointTime}\), then \(\timestep^p \vectorField_{\nnParams}^{[p]}(\midpoint)\) provides the exact value of the approximation error of the expansion.
In other words, if \(\midpoint\) were known, \eqref{eq:taylor_lagrange_expansion} provides an exact expression for the integral \(\state_{t_i} + \int_{t_i}^{t_{i+1}} \vectorField_{\nnParams}(\state_{s}) ds\).

While no closed form expression for the midpoint \(\midpoint\) exists, we propose to learn to predict these values given the state \(\state(\timeval_i)\), initial time \(\timeval_i\), and the time step \(\timestep\).
However, learning to predict the midpoint directly is a challenging problem in general.
% In particular, without putting any restrictions on the predicted values of \(\midpoint\), 
We instead propose to use the result of Theorem \ref{thm:expression-midpoint}, which provides a closed-form expression for the midpoint \(\midpoint\) in terms of some unknown term \(\midpointUnknownTerm \in \stateSpace\), to simplify the task of learning to predict \(\midpoint\).

\begin{theorem}[Simplified Midpoint Expression]\label{thm:expression-midpoint}
    If $\vectorField_{\nnParams}$ is a Lipschitz-continuous function, then the midpoint time \(\midpointTime\) of the Taylor-Lagrange expansion \(\taylorLagrange_{\nnParams}(\state, \timeval_{i}, \timeval_{i+1})\) satisfies,
    \begin{equation}
        \timeval_{i} \leq \midpointTime \leq \timeval_{i+1}, \text{ and, } \label{eq:midpoint_time_simple}
    \end{equation}
    the midpoint value \(\midpoint \in \stateSpace\) satisfies 
    \begin{equation}
        \midpoint = \state + \midpointUnknownTerm(\state, \timestep) \odot  \vectorField_{\nnParams}(\state), \label{eq:midpoint-simple}
    \end{equation}
    % \begin{align}
    %     &\midpoint = \state(\timeval_i) + \midpointUnknownTerm(\state(\timeval_i), \timestep) \odot  \vectorField_{\nnParams}(\state(\timeval_i), \timeval_i), \label{eq:midpoint-simple}\\
    %     &\min \{ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}), \state(\timeval_{i}) \} \leq \midpoint_\nnParams(\state(\timeval_i), \timeval_{i+1}-\timeval_{i}) \leq \max \{ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}), \state(\timeval_{i}) \},\label{eq:midpoint-constr}
    % \end{align}
    where $\midpointUnknownTerm$ is some function mapping from the state \(\state\) and time step \(\timestep\) to \(\stateSpace\), and \(\odot\) denotes the element-wise multiplication operation.
\end{theorem}

% \begin{theorem}[Simplified Midpoint Expression]\label{thm:expression-midpoint}
%     If $\vectorField_{\nnParams}$ is a Lipschitz-continuous function, then the midpoint value $\midpoint$ of the Taylor-Lagrange expansion \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\) satisfies
%     \begin{equation}
%         \midpoint = \state(\timeval_i) + \midpointUnknownTerm(\state(\timeval_i), \timestep) \odot  \vectorField_{\nnParams}(\state, \timeval_i), \text{ and, } \label{eq:midpoint-simple}
%     \end{equation}
%     \begin{equation}
%         \min \{\state, \taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1}) \} \leq \midpoint \leq \max \{\state,  \taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\},\label{eq:midpoint-constr}
%     \end{equation}
%     % \begin{align}
%     %     &\midpoint = \state(\timeval_i) + \midpointUnknownTerm(\state(\timeval_i), \timestep) \odot  \vectorField_{\nnParams}(\state(\timeval_i), \timeval_i), \label{eq:midpoint-simple}\\
%     %     &\min \{ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}), \state(\timeval_{i}) \} \leq \midpoint_\nnParams(\state(\timeval_i), \timeval_{i+1}-\timeval_{i}) \leq \max \{ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}), \state(\timeval_{i}) \},\label{eq:midpoint-constr}
%     % \end{align}
%     where $\midpointUnknownTerm$ is some function mapping from the state \(\state\) and time step \(\timestep\) to \(\stateSpace\), \(\odot\) denotes the element-wise multiplication operation, and the \(\min\) and \(\max\) operators are applied element-wise.
% \end{theorem}

% simplifies the problem of learning a function predicting the midpoint by

% To do so, we parameterize a neural network \(\midpoint_{\nnParamsMidpoint}\) that takes the values of \(\state\) and \(\timestep\) as input.

% To learn the midpoint value \(\midpoint\) of a particular Taylor-Lagrange expansion \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\), we parameterize a neural network \(\midpoint_{\nnParamsMidpoint}\) that takes the \(\state\) and the time step \(t_{i+1} - t_{i}\) as input, and predicts the value of \(\midpoint\).

% \paragraph{Simplify the Midpoint Learning.} 
% In this paper, we propose to learn the vector field $\vectorField_{\nnParams}$ alongside the midpoint value. To this end, we parameterize the midpoint value by a neural network having as inputs the state and the time step. We denote by $\midpoint_{\nnParams}$ the resulting function, and  we consider that the parameter $\nnParams$ contains both the parameters of the vectorfield $\vectorField$ and the midpoint $\midpoint$ parameterizations. To cope with the complexity of learning such a midpoint, we provide, in Theorem \ref{thm:expression-midpoint} a closed-form expression aiming at simplify its learning by reusing the knowledge of the vector field $\vectorField_{\nnParams}$.

% \begin{theorem}[Simplified Midpoint Learning]\label{thm:expression-midpoint}
%     If $\vectorField_{\nnParams}$ is a Lipschitz-continuous function, then the midpoint value $\midpoint(\nnParams)$ evaluated at $\state(\timeval_i)$ to predict $ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1})$ satisfies the following:
%     \begin{align}
%         &\midpoint_\nnParams(\state(\timeval_i), \timeval_{i+1}-\timeval_{i}) = \state(\timeval_i) + \midpoint^1_\nnParams(\state(\timeval_i), \timeval_{i+1}-\timeval_{i}) \vectorField_{\nnParams}(\state(\timeval_i), \timeval_i), \label{eq:midpoint-simple}\\
%         &\min \{ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}), \state(\timeval_{i}) \} \leq \midpoint_\nnParams(\state(\timeval_i), \timeval_{i+1}-\timeval_{i}) \leq \max \{ \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}), \state(\timeval_{i}) \},\label{eq:midpoint-constr}
%     \end{align}
%     where $\midpoint_\nnParams^1$ is the actual neural network that will be trained to predict the midpoint value through~\eqref{eq:midpoint-simple}, and the constraint in~\eqref{eq:midpoint-constr} ensures that the midpoint value lies between the current and next state values.
% \end{theorem}

% We provide a proof of Theorem~\ref{thm:expression-midpoint} in Appendix~\ref{}. Specifically, the theorem is obtained by using tools from interval Taylor-based reachability analysis. The formulation in~\eqref{eq:midpoint-simple} is derived from our explicit formula for the so-called \emph{apriori} enclosure: A set guaranteed to contain the next state value $\neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1})$ under some local Lipschitz bound knowledge. 

Theorem~\ref{thm:expression-midpoint} is obtained using tools from interval Taylor-Langrange based reachability analysis \cite{djeumou2021fly}.
More specifically, the equation given in \eqref{eq:midpoint-simple} is derived from explicit formulas for the so-called \emph{apriori} enclosure -- a set derived from the local Lipschitzness of \(\vectorField_{\nnParams}\) that is guaranteed to contain the value of \(\taylorLagrange^{\timestep}_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\).
The constraint in~\eqref{eq:midpoint_time_simple} ensures that the midpoint time \(\midpointTime\) lies between the center point and the evaluation point of the Taylor-Lagrange expansion.
A proof of Theorem~\ref{thm:expression-midpoint} is provided in the Appendix.

% \color{red}
% Besides, a stronger result in the proof of Theorem~\ref{thm:expression-midpoint} suggests that the resulting neural network $\midpoint^1_\nnParams$ is a function of only the Lipschitz bounds of $\vectorField_\nnParams$, the time step $\timeval_{i+1}- \timeval_{i}$, and a small value between $-1$ and 1 that depends on $\state(\timeval_i)$. Hence, the claim that \eqref{eq:midpoint-simple} is a simpler learning representation for the midpoint value.
% \color{black}

Given the result of Theorem \ref{thm:expression-midpoint}, we propose to parameterize the unknown function \(\midpointUnknownTerm_{\nnParamsMidpoint}(\cdot)\) using a neural network with parameters \(\nnParamsMidpoint\).
For notational simplicity, we use \(\midpoint_{\nnParamsMidpoint}(\state, \timestep)\) to denote the value of the right hand side of \eqref{eq:midpoint-simple} when \(\midpointUnknownTerm(\cdot)\) is approximated by \(\midpointUnknownTerm_{\nnParamsMidpoint}(\cdot)\).
Given the predicted midpoint value \(\midpoint_{\nnParamsMidpoint}(\state, \timestep)\) of the \(p^{th}\) order Taylor-Lagrange expansion \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\), we estimate the expansion's approximation error as \(\timestep^{p}\vectorField_{\nnParams}^{[p]}(\midpoint_{\nnParamsMidpoint}(\state, \timeval_i, \timestep))\).
% when computing the right hand side of \eqref{eq:taylor_lagrange_expansion}.

\input{algs/evaluation_alg}

\subsection{Bounding the Error of the Taylor-Lagrange Integrator}
% \paragraph{Accuracy of Taylor-Lagrange with Learned Midpoint.}
We seek to bound the error on a \(p^{th}\) order Taylor-Lagrange expansion which uses a learned midpoint value predictor \(\midpoint_{\nnParamsMidpoint}\).
Such an error bounds straightforwardly depends on how well \(\midpoint_{\nnParamsMidpoint}\) approximates the true midpoint \(\midpoint\), as described in Theorem \ref{thm-approximation-error}.
% We seek to provide an approximation error bound on a $p^{th}$ order Taylor-Lagrange expansion with learned midpoint value $\midpoint_{\nnParams}$. Such error straightforwardly depends on how well $\midpoint_{\nnParams}$, defined in~\eqref{eq:midpoint-simple}, can approximate the midpoint $\midpoint$. 
A proof of Theorem~\ref{thm-approximation-error} is provided in the Appendix.

\begin{theorem}[Integration Accuracy]\label{thm-approximation-error}
    If the learned midpoint predictor \(\midpoint_{\nnParamsMidpoint}\) is a $\mathcal{O}(\eta)$ approximator to the midpoint value $\midpoint$ of the Taylor-Lagrange expansion of \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\), then $\| \state(\timeval_{i+1}) - \taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1}) \| \leq c \eta \timestep^{p+1}$ for some $c > 0$ that depends on the Lipschitz constant of $\vectorField_{\nnParams}$.
\end{theorem}   

% \begin{theorem}[Integration Accuracy]\label{thm-approximation-error}
%     If the trained neural network $\midpoint_{\nnParams}$ given in~\eqref{eq:midpoint-simple} is a $\mathcal{O}(\eta)$ approximator of the unknown midpoint value $\midpoint$ of the Taylor-Lagrange expansion of $\vectorField_{\nnParams}$, then the local truncation error is $\mathcal{O}((\timeval_{i+1}-\timeval_{i})^{p+1} \eta)$, i.e., $\| \state(\timeval_{i+1}) - \neuralODE_{\nnParams}(\state, \timeval_i, \timeval_{i+1}) \| \leq c \eta (\timeval_{i+1}-\timeval_{i})^{p+1}$ for some real positve value $c$ that depends on the Lipschitzness of $\vectorField_{\nnParams}$.
% \end{theorem}   


%%%%%%%%%%%%%%%%%%%%%
% We note that trying to use \(\midpoint_{\nnParamsMidpoint}(\state, \timeval_i, \timestep)\) to compute \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\) results in a circular dependency; the value of \(\midpoint_{\nnParamsMidpoint}\) relies on the value of \(\taylorLagrange_{\nnParams}\), however, \(\midpoint_{\nnParamsMidpoint}\) is simultaneously being used to compute the value of \(\taylorLagrange_{\nnParams}\).
% In order to get around this issue and to properly use the estimated approximation error \(\midpoint_{\nnParamsMidpoint}\) to compute \(\taylorLagrange_{\nnParams}\), we proceed as follows.
% We first compute \(\taylor_{\nnParams}(\state, \timeval_i, \timeval_{i+1}) = \state + \sum_{i=1}^{p-1} \timestep^{l} \vectorField_{\nnParams}^{[l]}(\state, \timeval_i)\), i.e. the truncated Taylor expansion of \(\vectorField_{\nnParams}\) without the approximation error term.
% We then compute the value of \(\midpoint_{\nnParamsMidpoint}(\state, \timeval_i, \timestep)\) while using \(\taylor_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\) instead of \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\) to define the inequality constraints in \eqref{eq:midpoint-constr}.
% Finally, we substitute \(\midpoint_{\nnParamsMidpoint}(\state, \timeval_i, \timestep)\) into \eqref{eq:taylor_lagrange_expansion} to compute the value of \(\taylorLagrange_{\nnParams}(\state, \timeval, \timeval_{i+1})\).
%%%%%%%%%%%%%%%%%%%%%%%

% Intuitively, consider a one dimensional ODE and assume for the sake of the illustration that $\timeval_{i+1} - \timeval_{i}$ is sufficiently small such that $\state(\timeval_{i+1}) = \state(\timeval_i) + (\timeval_{i+1} - \timeval_{i}) \vectorField_{\nnParams}(\state(\timeval_i), \timeval_i)$ is a good approximation of the next state value. Then, a simple and expressive parameterization of the midpoint that uses the knowledge of the vector field is given by $\state(\timeval_i) + \alpha \vectorField_{\nnParams}(\state(\timeval_i), \timeval_i)$, for some real number $\alpha = \midpoint^1$.

% \textcolor{blue}{Some details about the loop issue on the constraint here and the fact that in scenario where the data are directly over state values, we can have explicit (non-dependent on the unknown next state) constraints (7)}

\subsection{Training the Taylor-Lagrange Networks}

Using the methods described in \S \ref{sec:TL_numerical_integration_of_neural_ode} and \S \ref{sec:learning_the_midtpoint}, we compute the output of the neural ODE \(\neuralODE_{\nnParams}(\state, \initTime, \predictionTime)\) by iteratively using \(\taylorLagrange_{\nnParams}(\state, \timeval_i, \timeval_{i+1})\) to numerically integrate \(\vectorField_{\nnParams}\) over the time intervals \([t_i, t_{i+1}]\).
Given a dataset \(\dataset = \{(\state^j, \initTime^j, \predictionTime^j, \trueNextState^j)\}_{j=1}^{|\dataset|}\), where each datapoint consists of an initial state \(\state^j\), an initial time \(\initTime^j\), a prediction time \(\predictionTime^j\), and the value of the state at the prediction time \(\trueNextState^j\), we simultaneously train \(\nnParams\) and \(\nnParamsMidpoint\) via the optimization problem given in \eqref{eq:loss_opt_problem}.

\begin{equation}
\begin{split}
    \min_{\nnParams, \nnParamsMidpoint}  & \sum_{(\state^j, \initTime^j, \predictionTime^j, \trueNextState^j) \in \dataset} \left[
    \loss(\neuralODE_{\nnParams}(\state^j, \initTime^j, \predictionTime^j), \trueNextState^j) \right. \\
    & \left. + \penaltyCoef * \penaltyTerm(\state^j, \initTime^j, \predictionTime^j) + \regularizationCoef * \regTerm(\state^j, \initTime^j, \predictionTime^j)
    \right]
\end{split}   
\label{eq:loss_opt_problem}
\end{equation}

Here, \(\loss(\neuralODE_{\nnParams}(\state, \initTime, \predictionTime))\) is some loss function defined on the outputs of the neural ODE, and \(\penaltyCoef, \regularizationCoef \geq 0\) are scalar parameters.
\(\penaltyTerm(\state, \initTime, \predictionTime)\) is a function measuring of the extent to which the constraints in \eqref{eq:midpoint-constr} are violated throughout the numerical integration of \(\vectorField_{\nnParams}\) from \(\initTime\) to \(\predictionTime\).
We note that the inclusion of \(\penaltyTerm\) in \eqref{eq:loss_opt_problem} penalizes the optimization objective if the neural network \(\midpoint_{\nnParamsMidpoint}\) learns to outputs midpoint values that are infeasible; the midpoint should always take values between the expansion point and the evaluation point of the Taylor series.
% 
% This constraint helps to prevent the model from learning far away points thus inflating the error term in order to overfit the training data.
% \(\penaltyCoef, \regularizationCoef \geq 0\) are scalar parameters.
\begin{equation}
\begin{split}
    \penaltyTerm(\state, & \initTime, \predictionTime) = \sum_{i=0}^{\numIntervals} \Bigl[ l_{hinge} \Bigl( \midpoint_{\nnParamsMidpoint}(\hat{\state}_i, \timeval_i, \timestep) \Bigr. \Bigr. \\
    & \quad \quad \quad \quad \quad \quad \quad \Bigl. - \max\{\hat{\state}_i, \taylorLagrange_{\nnParams}(\hat{\state}_i, \timeval_i, \timeval_{i+1})\} \Bigr)^2 \\
    & + l_{hinge} \Bigl( \min\{\hat{\state}_i, \taylorLagrange_{\nnParams}(\hat{\state}_i, \timeval_i, \timeval_{i+1})\} \Bigr.\\
    & \quad \quad \quad \quad \quad \quad \quad \quad \quad \Bigl. \Bigl. - \midpoint_{\nnParamsMidpoint}(\hat{\state}_i, \timeval_i, \timestep)\Bigr)^2 \Bigr]
\end{split}
\label{eq:penaltyTerm}
\end{equation}
% 
Meanwhile, \(\regTerm(\state, \initTime, \predictionTime)\) measures the magnitude of the approximation errors accumulated during numerical integration.
Intuitively, this penalty term ensures that the predicted approximation error values will remain small, preventing the neural network \(\midpoint_{\nnParamsMidpoint}\) from overfitting the training data.
% which is helpful to prevent the neural ODE from using \(\midpoint_{\nnParamsMidpoint}\) from overfitting the training data.
% of the numerical estimator to be as small as possible.
% 
\begin{equation}
    \regTerm(\state, \initTime, \predictionTime) = \sum_{i=0}^{\numIntervals - 1} || \timestep^p \vectorField_{\nnParams}^{[p]}(\midpoint_{\nnParamsMidpoint}(\hat{\state}_i, \timeval_i, \timestep)) ||_2^2
    \label{eq:reg_term}
\end{equation}
% 
In both of the above equations, \(\hat{\state}_i\) denotes integrator-estimated intermediate state value at time \(t_i\).
% The inclusion of this penalty term helps constrain the model of \(\midpoint_{\nnParamsMidpoint}\), preventing it from learning unreasonable values in order to overfit the training data by controlling the 

% \textbf{Regularizing the Approximation Error}\\

% \textcolor{blue}{In order to avoid overfitting (need to explain), we seek for solutoons for which the remainder $(\timeval_{i+1}-\timeval_{i})^{p} \vectorField_{\nnParams}^{[p]}(\midpoint)$ is small. So we penalize.}

% \paragraph{How to Train Neural ODEs using Taylor-Lagrange.}
% 
% \textcolor{blue}{Details on the training algorithms (maybe the algorithm itself)}


% \textcolor{blue}{A table summarizing the number of function evaluation and accuracy of p-order RK, p-order truncated, and p-order Tayla}

% \textcolor{blue}{Some notation needs to be defined: Lipschitz-continuous, sufficiently-smooth, Big $\mathcal{O}$ symbols etc...}


\input{algs/training_alg}

==> tex/05_numerical_experiments_v1.tex <==
\section{Numerical Experiments}
\label{sec:numerical_experiments}

% \color{red}
% \begin{itemize}
%     \item Integration of known stiff dynamics.
%     \begin{itemize}
%         \item The main message: Our proposed method for learning the midpoint value is empirically justified.
%         \item Plots showing that we are effectively learning the midpoint (this will be a plot of the midpoint (and predicted midpoint) value as a function of \(\Delta t\).
%         Note that we can make such a plot for the case of linear dynamics because we can derive analytic expressions for the midpoint value.
%         \item Comparisons of the prediction error with fixed-step RK methods, adaptive time-step methods, hypersolver (which learns the whole remainder instead of using nice expressions to simplify learning), and with truncated taylor expansions without taylor expansions.
%         This will highlight the gain in accuracy that estimating the midpoint gives.
%         This also highlights the fact that our method to learn the midpoint is better than that of hypersolver, because we use the midpoint theorem.
%         \item Plots of computation time vs \(\Delta t\) to highlight the fact that we beat adaptive time-step methods in terms of computation time.
%     \end{itemize}

%     \item Learning some dynamical system.
%     \begin{itemize}
%         \item The main message: that our two-step procedure for learning the dynamics and the midpoint works.
%         \item Plot the loss as a function of training steps.
%         \item Plot the evolution of the trajectory.
%     \end{itemize}

%     \item Supervised classification.
%     \begin{itemize}
%         \item 
%     \end{itemize}

% \end{itemize}
% \color{black}

We demonstrate the effectiveness of TL-NODE through several numerical experiments: the numerical integration of known dynamics, the learning of unknown dynamics, a supervised classification task, and a density estimation task.
Additional experimental details and results are included in the supplementary material.
% For brevity, in this section we denote the neural ODE trained with our proposed Taylor-Lagrange expansion method as TLN.

\begin{figure}[t]
\centering
\input{figs/stiff_dynamics/plot_stiff_dynamics}
\caption{Numerical integration of known stiff dynamics. We compare the proposed approach (TL-NODE) to fixed-step RK4, adaptive-step RK4, and Hypersolver \cite{Poli2020HypersolversTF}. Top left: Time taken to numerically integrate 100 initial values over 8 integration time steps, as a function of the size of the time step. Top right: Visualization of the integrated trajectories in the state space, \(\timestep = 0.001\). Bottom left: Mean error accumulated over 8 integration time steps, measured across 100 randomly sampled initial points. Bottom right: Geometric mean of the numerical integration error as a function of time, measured across 100 randomly sampled initial points, \(\timestep = 0.001\).}
\label{fig:known_dynamics_results}
\end{figure}

\subsection{Integration of Known Dynamics}
\label{sec:numerical_integration_known_dynamics}

To examine the accuracy and robustness of the midpoint prediction network \(\midpoint_{\nnParamsMidpoint}(\cdot)\), we begin by presenting the results of applying the proposed Taylor-Lagrange numerical integration method to a two-dimensional system with known stiff dynamics.
% To demonstrate the numerical accuracy and the fast evaluation times of the proposed approach, we test the integrator on a system with known stiff dynamics.
More specifically, we use the proposed Taylor-Lagrange approach to integrate the ODE \(\dot{\state} = A \state\), where \(\state \in \mathbb{R}^2\) and \(A \in \mathbb{R}^{2 \times 2}\) has eigenvalues \(\lambda_1 = -1\) and \(\lambda_2 = -1000\).

We note that the dynamics function \(\vectorField(\cdot)\) is known, so there is no need to parameterize the system dynamics using a neural network \(\vectorField_{\nnParams}(\cdot)\).
However, we may still apply the method outlined in \S \ref{sec:training_tlnode} to train \(\midpoint_{\nnParamsMidpoint}\) to predict the approximation error values of the Taylor-Lagrange expansions used for numerical integration of \(\vectorField(\cdot)\).
Furthermore, the true value of the midpoint \(\midpoint\) can be obtained analytically, allowing for a direct empirical analysis of the performance of the proposed midpoint prediction network.
% However, we still use the method outlined in \S \ref{sec:learning_the_midtpoint} to train a model \(\midpoint_{\nnParamsMidpoint}\) to predict the approximation error values of the Taylor-Lagrange expansions used for numerical integration.

\textbf{Experimental setup.} We parameterize the unknown term \(\midpointUnknownTerm_{\nnParamsMidpoint}\) in \eqref{eq:midpoint-simple} as a fully connected MLP with hyperbolic tangent activation functions and two hidden layers of 32 units each.
The dataset used to train \(\midpointUnknownTerm_{\nnParamsMidpoint}\) consists of 100 separate trajectories beginning from initial states that are randomly sampled from within a bounded region of the state space. 
Each trajectory is integrated for \(\predictionTime=10\) seconds, for varying sizes of the integration time step \(\timestep\).
The testing dataset consists of 100 trajectories beginning from initial states that are randomly sampled from a separate region of the state space.
% The labels of all datapoints are obtained from the analytical solution to the true dynamics.
% To method is tested on a dataset generated by sampling 100 
The network is optimized using ADAM \cite{kingma2014adam} with a learning rate of \(1e-3\).

% \begin{figure*}
% \centering
% \input{figs/stiff_dynamics/plot_stiff_dynamics}
% \caption{Numerical integration of known stiff dynamics.
% We compare the proposed approach (TL-NODE) to fixed-step RK4, adaptive-step RK4, and Hypersolver \cite{Poli2020HypersolversTF}.
% Top left: Time taken to numerically integrate 100 initial values over 8 integration time steps, as a function of the size of the time step.
% Top right: Visualization of the integrated trajectories in the state space, \(\timestep = 0.001\).
% Bottom left: Mean error accumulated over 8 integration time steps, measured across 100 randomly sampled initial points.
% Bottom right: Geometric mean of the numerical integration error as a function of time, measured across 100 randomly sampled initial points, \(\timestep = 0.001\).}
% \label{fig:known_dynamics_results}
% \end{figure*}

% \color{red}
% % Add the details of the neural network setup used for this experiment.
% Add the details of the training setup used for this experiment. How many training datapoints? What optimization algorithm was used? What order of Taylor-Lagrange expansion do we use?
% \color{black}

For comparison, we include the results of a fixed-step RK4 method, an adaptive-step RK4 method, and the \textit{Hypersolver} method.
The Hypersolver method is setup as proposed in \cite{Poli2020HypersolversTF}, with the Hypersolver neural network following an identical structure to the network used to parameterize \(\midpointUnknownTerm_{\nnParamsMidpoint}\).
The tolerance parameters \(rtol\) and \(atol\) of the adaptive-step RK4 integrator are both set to 1.4e-8.
As a further point of comparison, we additionally plot the result of using the truncated Taylor expansion for integration, without including the learned approximation error term.

\textbf{Discussion of the results.} Figure \ref{fig:known_dynamics_results} illustrates the numerical integration results.
% We observe that the proposed approach achieves computation times that are faster than the adaptive step-size method, while also enjoying lower integration error than all other baseline approaches.
We observe that TLN enjoys lower integration error than all of the baseline methods except for adaptive-step RK4.
However, adaptive-step RK4 requires computation times that are roughly an order of magnitude higher than that of our method.
We additionally observe that while the Hypsersolve method requires similar computation time to TLN, the error of its numerical integration results are an average of are two orders of magnitude higher.
Finally, the integration error of the truncated Taylor expansion method is also two orders of magnitude higher than that of TLN. 
These results demonstrate the effectiveness of the proposed approach for learning to predict the approximation error term in the Taylor-Lagrange expansion. This learned approximation error term is the only difference between TLN and the truncated Taylor expansion method.
% Furthermore, we note that Hypersolver also attempts to 

\subsection{Learning Unknown Dynamics}

% The proposed approach enjoys lower integration error than all of the baseline methods except for adaptive-step RK4.
% However, adaptive-step RK4 requires computation times that are roughly an order of magnitude higher than that of our method.
% We additionally observe that while the Hypsersolve method requires similar computation times with our method, 

==> tex/99_todo_list.tex <==
TODO list:
\begin{itemize}

    \item \st{Re-phrase everything in terms of predictor corrector schemes.}
    \begin{itemize}
        \item \st{Add predictor-corrector literature to the related work.}
    \end{itemize}

    
    \item \st{Implicit constraints on midpoint value.}
    \begin{itemize}
        \item \st{Change Theorem 1 (simplified midpoint expression)}
    \end{itemize}
    
    \item \st{Moving away from training midpoint and neural ODE all together (with regularization on midpoint predictions). Instead holding midpoint fixed while training neural ODE, and then periodically fixing the predictor and training the corrector.}

    \item Add intro block diagram and taylor expansion visualization figure.
    \begin{itemize}
        \item Add some results to the intro as well.
    \end{itemize}
    
    \item Add a running example (stiff linear dynamics) to the paper. The point is to help illustrate what the midpoint is, what values it can take, and how experimentally we match it. This example will also help to demonstrate how we are outperforming RK4 and first-order Euler and making good compromises between accuracy and speed.
    
    \item \st{Add an algorithm.}

    \item Examples
    \begin{itemize}
        \item Integration of known stiff dynamics.
        \begin{itemize}
            \item Illustration of computation time vs accuracy.
        \end{itemize}
        
        \item Supervised Classification
        \begin{itemize}
            \item Illustration of comparable accuracy to baselines, while having much lower number of function evaluations.
            \item Include a table showing computation time for training convergence.
        \end{itemize}
        
        \item FFJORD examples
    \end{itemize}
\end{itemize}
\newpage
